Helfrich cylinders -- instabilities, bifurcations and amplitude equations

Combining local bifurcation analysis with numerical continuation and bifurcation methods we study bifurcations from cylindrical vesicles described by the Helfrich equation with volume and area constraints, with a prescribed periodicity along the cylindrical axis. The bifurcating solutions are in two main classes, axisymmetric (pearling), and non-axisymmetric (coiling, buckling, and wrinkling), and depending on the spontaneous curvature and the prescribed periodicity along the cylinder axis we obtain different stabilities of the bifurcating branches, and different secondary bifurcations.

==> c075.tex <==
%\input{c1f1}
\subsection{Outlook: $c_0=0.75$}\label{cpsec}
Lastly, following Fig.\ref{neigs}(e) we consider 
$c_0>1/2$, specifically $c_0=0.75$ for which 
$\CC_L$ is never stable if $L\ge 2\pi $ ($k_1\le 1$, say), and    
branches as before still bifurcate from $\CC_L$, 
but not at loss of stability of $\CC_L$. 
Hence they can also still be described by AEs as before, but they cannot 
be stable close to bifurcation, and we can only expect stable ``patterns'' 
at $O(1)$ amplitude. This is more difficult than 
the analysis and numerics so far, and hence here we only give 
an outlook on some interesting (numerical) results we obtain, 
again for a rather small length $L=10$ of the cylinder, and 
leave more systematic and detailed studies to later work. 

\input{c1f1}

Figure \ref{c1f1} shows the BD of $k_1\approx 0.628$ pearling 
(A, blue) and $k_2\approx 1.257$ pearling (C, light blue), 
which are both unstable at bifurcation as they must, and 
moreover are unstable throughout, 
and addtionally an $O(1)$ amplitude pearling branch (P, red), 
where P$_2$ is obtained from DNS  starting 
near A$_1$ (panel (c)). In summary, we see a number of new effects which 
strongly suggest further study, but here we restrict to the following comments.

$\bullet$ We stop the continuations shortly after A$_3$, shortly 
after C, and shortly after P$_1$ as further continuations there 
require excessive mesh--adaptations. We can continue significantly 
beyond P$_3$, but our main region of interest is near $v=1$. 
There are bifurcations on the blue branches which break the 
rotational symmetry, but we restrict to presenting axisymmetric branches. 

$\bullet$ The $k_1$ pearling branch A shows two folds in $v$, 
the first at $v_{f,1}\approx 1.045$, the second at 
$v_{f,2}\approx 0.98$. In particular, between A$_1$ and A$_2$ 
it goes through $v=1$ again, while keeping the area $\CA$ 
constant throughout. This is not a contradiction to the fact 
that normal variations to $\CC_L$ that fix $\CA$ and $\CV$ 
locally do not exist; the passage through $v=1$ here 
corresponds to a non--small normal variation. 

$\bullet$ The folds on the 
A branch naturally call for fold continuation in $c_0$, in 
particular for decreasing $c_0$ as for $c_0<1/2$ we do not see 
folds on the analogous A branches. We believe that they vanish 
at some $c_0>1/2$ as the blue swallowtail shrinks and the folds 
collide, but this remains to be studied. 
%Presently we can only do this in a very inefficient way largely based on numerical Jacobians for the extended system for the fold continuation, and this needs to be improved first. The same applies to branch point continuation as another relevant two--parameter problem. 

$\bullet$ The flow in (c) starts at A$_1$ with a small pertubation 
in direction of the most unstable eigenvalue; 
A$_1$ is below the fold, and there is exactly one 
positive eigenvalue $\mu\approx 0.2$. In any case, 
the results of flow experiments seem rather robust wrt 
the choice of the initial conditions (choice of steady state 
and perturbation), i.e., we always ``land'' on the P branch, 
though naturally at different $v$ and $\lam_2$, or analoga 
of the P branch at different area $\CA$. In the particular 
case shown, the perturbation of A$_1$ yields a relative 
change of $\CV$ of order $10^{-3}$, and a relative change of 
$\CA$ of order $10^{-4}$. (The initial perturbation 
{\em linearly} conserves $\CA$ and $\CV$, i.e., 
is tangential to the constraint manifold, but 
for any finite perturbation we must expect a (nonlinear) 
change of $\CA$ and $\CV$. However, the change in $\CA$ is 
so small that we ignore it and keep the normalization of 
$E$ in \reff{enorm} by the original $\CA$.) 

$\bullet$ The last plots in (c) suggest almost steady states for $t>20$, 
and we use the solution at $t=20.95$ as an initial guess for 
Newton's method for the steady problem. This indeed takes us to the 
(spectrally) stable steady state P$_2$, and continuing 
from here to larger/smaller $v$ yields the red branch. 

$\bullet$ It is remarkable that the P branch with two pearls of different 
sizes  is stable, that along the branch the pearls change their relative 
sizes (different from the primary pearling branches, where only 
the amplitude changes), 
and that in fact P$_2$ attracts (perturbations of) A$_1$.  
However, this is partly a finite size effect, because some stability 
of the P branch is lost when 
repeating the experiment from Fig.\ref{c1f1} on larger domains, 
e.g., $L=20$. In this case, initial conditions for numerical flows 
must be chosen more carefully, namely closer to $v=1$ to reach the analogue 
of the P branch (4 pearls on $L=20$), and continuation of the P branch 
then shows a loss of stability (wrt to still axially symmetric solutions) 
away from $v=1$. 
We plan to study in particular these effects 
in a systematic way in future work. %\hfill\mbox{{}}

$\bullet$ Shape wise (compare P$_1$ and C in (d)) it seems possible 
that the P branch connects to the C branch in a period--doubling 
bifurcation, but samples  P$_1$ and C are at rather different values of 
$\lam_{1,2}$. In our preliminary experiments so far we could not 
identify to what  other branches the P branch connects, and again we 
leave this for future work. 



%\input{c1f1}


  

==> c0f2.tex <==
\begin{figure}[ht]
  \begin{center}
\btab{l}{
\btab{ll}{
{\small (a),  from Fig.\ref{c00f}A$_2$}\\[-0mm]
 \hs{-4mm}\ig[height=0.24\tew]{c0f2/0f1-0} 
\hs{1mm}\ig[height=0.24\tew]{c0f2/0f1-e} 
&\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f1E}
\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f1l2}
\hs{-0mm}\ig[height=0.24\tew]{c0f2/0f1A}\\[-0mm]
{\small (b),  from Fig.\ref{c00f}B}\\[-0mm]
\hs{-4mm}\ig[height=0.24\tew]{c0f2/0f6-0} 
\hs{-1mm}\ig[height=0.24\tew]{c0f2/0f6-e} 
&\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f6E}
\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f6lt}
\hs{-0mm}\ig[height=0.24\tew]{c0f2/0f6A}
\\[-0mm]
{\small (c$_1$), from Fig.\ref{c00f}C,  perturbation by \reff{flp1}}\\
%, flow to stable wave}\\
\hs{-4mm}\ig[height=0.24\tew]{c0f2/0f10-0} 
\hs{-1mm}\ig[height=0.24\tew]{c0f2/0f10-e} 
&\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f10E}
\hs{-2mm}\ig[height=0.24\tew]{c0f2/0f10lt}
\hs{-0mm}\ig[height=0.24\tew]{c0f2/0f10A}
\\[-0mm]
{\small (c$_2$), from Fig.\ref{c00f}C, perturbation by \reff{flp2}}\\
%, flow to nearby coil}\\
\hs{-4mm}\ig[height=0.24\tew]{c0f2/f11b0} 
\hs{-1mm}\ig[height=0.24\tew]{c0f2/f11be} 
&\hs{-2mm}\ig[height=0.24\tew]{c0f2/f11bE}
\hs{-0mm}\ig[height=0.24\tew]{c0f2/f11blt}
\hs{-0mm}\ig[height=0.24\tew]{c0f2/0f11bA}
\\[-0mm]
 }
}
\vs{-0mm}
  \end{center}
  \caption{{\small Numerical flows from perturbations of states from 
Fig.\ref{c00f}; initial and 'final' state, and evolution of $E$, $\lam_{1,2}$ 
(only $\lam_2$ in (a) and (c$_2$)), and deviations from initial area and volume; 
very slow evolution in (c$_2$). \label{c0f2}}}
\end{figure}


==> c1f1b1.tex <==
\begin{figure}[ht]
  \begin{center}
\btab{l}{
\btab{ll}{{\small (a)}&{\sm (b)} \\
\hs{-4mm}\ig[height=0.32\tew]{ff/bdE075} 
\hs{-2mm}\ig[height=0.32\tew]{ff/bdl075}  
&\hs{-1mm}\ig[height=0.3\tew]{ff/A1} \hs{-1mm}\ig[height=0.3\tew]{ff/A2} 
 \hs{-1mm}\ig[height=0.3\tew]{ff/A3} 
}\\
{\small (c)}\\
\hs{-3mm}\ig[height=0.17\tew]{ff/C} \hs{-1mm}\ig[height=0.17\tew]{ff/P1} 
 \hs{-1mm}\ig[height=0.17\tew]{ff/P2} \hs{-1mm}\ig[height=0.17\tew]{ff/P3} 
}
\vs{-0mm}
  \end{center}
  \caption{{\small Selected branches for $c_0=0.75$, $L=10$. 
(a) Energy $E$ over 
reduced volume $v$, and $\lam_1$ over $\lam_2$. (b) Samples from 
primary pearling (blue branch in (a)) all unstable. (c) Sample 
from $m=2$ pearling (light blue), and samples from stable red 
pearling branch, with $P_2$ generated from DNS starting at $A_1$. 
\label{c1f1}}}
\end{figure}


==> c1f2.tex <==
\begin{figure}[ht]
  \begin{center}
\btab{l}{
\hs{-3mm}\ig[height=0.28\tew]{ff/Ef} \hs{-1mm}\ig[height=0.28\tew]{ff/l12f} 
 \hs{1mm}\ig[height=0.23\tew]{ff/f1} \hs{-1mm}\ig[height=0.23\tew]{ff/f2} 
 \hs{-1mm}\ig[height=0.23\tew]{ff/f3c} \hs{-0mm}\ig[height=0.23\tew]{ff/f4} 
}
\vs{-0mm}
  \end{center}
  \caption{{\small flow 
\label{c1f2}}}
\end{figure}


==> cmf1.tex <==
\begin{figure}[H]
  \begin{center}
\btab{l}{
\btab{ll}{{\small (a$_1$)}&{\sm (a$_2$)}\\
\hs{-4mm}\ig[height=0.33\tew]{cm1f/bdE} 
& \hs{-4mm}\ig[height=0.33\tew]{cm1f/bdla} 
%&\ig[width=0.25\tew]{cm1f/A}\hs{4mm}\ig[width=0.25\tew]{cm1f/B}
}\\
{\small (b)}  \\[-1mm]
\ig[width=0.16\tew]{cm1f/A}\hs{-0mm}\ig[width=0.16\tew]{cm1f/B}
\ig[width=0.16\tew]{cm1f/C}\hs{-0mm}\ig[width=0.16\tew]{cm1f/D1}
\hs{-0mm}\ig[width=0.16\tew]{cm1f/D2}\hs{-0mm}\ig[width=0.16\tew]{cm1f/E}\\
{\small (c)}\\
\ig[width=0.29\tew]{amp/m1wv} \ig[width=0.29\tew]{amp/m1wlam} 
\ig[width=0.29\tew]{amp/m1wlamlam} 

} 
\vs{-0mm}
  \end{center}
  \caption{{\small Basic BD (a) for $c_0=-1$, $L=10$, and samples (b).  
(a$_1$) Energy $E$ over $v$; (a$_2$) $\lam_1$ over 
$\lam_2$ for the wrinkling D and 'embedded oblates' E. (c) 
Comparison with AE prediction for primary wrinkling.  \label{cmf1}}}
\end{figure}


==> husiammod.tex <==
\makeatletter
\renewcommand*\@ptsize{2}
\let\small\relax \let\footnotesize\relax \let\scriptsize\relax
\let\tiny\relax \let\large\relax \let\Large\relax \let\LARGE\relax
\let\huge\relax \input{size1\@ptsize.clo} 
\makeatother
\makeatletter
\@twosidefalse
\makeatother
\usepackage[top=25mm,left=20mm]{geometry}\textwidth16.7cm\textheight23cm

==> inex.tex <==
\begin{figure}[ht]
%\bce
\btab{lllll}{{\small (a)}& {\small (b)}  \\
\hs{0mm}\ig[width=0.25\tew]{intex/braV}&
\raisebox{4mm}{ \hs{-5mm}\ig[width=0.25\tew]{intex/0b1-23}}& 
\raisebox{4mm}{ \hs{-5mm}\ig[width=0.25\tew]{intex/0b2spo-21}} & 
\raisebox{4mm}{ \hs{-5mm}\ig[width=0.25\tew]{intex/0b2st-25}} 
\\

}
%\ece 
\vs{-6mm}
\caption{\small{Bifurcation diagram (a) of \reff{helf1} for the case $L=10$ and $c_0=0$. With sample solutions in (b) for the first bifurcation {\tt 0-BP1} in dark red to an axisymmetric branch. Then two branches bifurcating from {\tt 0-BP2} to the unstable spot like on the orange and stable spiral (strip like) solutions on the green branch. }  
\label{intexfig1}}
\end{figure}


==> numex.tex <==
\section{Numerical examples} \label{numex}
We now use numerical continuation and bifurcation methods 
to corroborate the local results from 
\S\ref{aesec}, and to extend them to a more global picture. 
This includes some secondary bifurcations with interesting stable 
shapes away from the straight cylinder. The numerical setup follows 
the stability analysis in \autoref{stabrange} and \S\ref{redeq}. 
Namely, we fix a period $L$ (e.g., $L=10$, $L=15$ or $L=30$, see 
also Remark \ref{carem}),  and the area $\CA=\CA(X)$, and 
initially use $\lam_2$ as the primary bifurcation parameter 
and $\lam_1$ and $\CV(X)$ as secondary (dependent) parameters. 
The linearized stability of the solutions, however, is then computed for 
fixed $\CA(X)$ and $\CV(X)$ while $\lam_1$ and $\lam_2$ are free parameters. 
Due to the radius-length scaling invariance of the Helfrich energy \reff{helfen} and the area and volume constraint in the dynamical 
problem, it is useful to introduce the reduced volume  
\hueq{\label{redvol} v=\CV(X)/\CV_0,} 
 where $\CV_0$ is the volume of the straight cylinder with the same $\CA(X)$, 
compare \cite{JSL93}, and we normalize the energy 
\hueq{\label{enorm}
\tilde E(X)=\frac 1 \CA \int_X (H-c_0)^2\dd S.} 
Also for our numerics we focus on the three exemplary cases 
\hugast{
\text{(a) $c_0=0$,\quad (b) $c_0=-1$, \quad and (c) $c_0=0.48$}
} 
from Fig.\ref{neigs}, and mostly 
we use $L=10$. For (a) and (b) 
this is no significant restriction as in these cases the primary 
bifurcations (to pearling, buckling and coiling in (a), and to pearling and 
wrinkling in (b)) are of long wave type for any (sufficiently large) $L$, 
i.e., a different $L$ gives the same types of primary bifurcations with 
different axial (maximal) periods $L$ (and the wrinkling is independent of $L$). 
However, for (c) and sufficiently large $L$ (preferably an integer 
multiple of the critical period $\ell\approx 7.5$) we have a 
finite wave number pearling instability. Thus, besides the case $L{=}10$ 
(for comparison with (a) and (b)), for (c) we shall consider different 
multiples of 7.5 for $L$, namely $L{=}15, L{=}30$, and $L{=}45$, allowing 
2, 4, and 6, pearls on the primary branch. The influence of $L$ 
will then be the behavior of this branch away from bifurcation, 
which loses stability in a bifurcation to a single pearl branch, 
and this BP moves closer to the primary BP with increasing $L$. 
This is further discussed in \S\ref{dsec}. 
\huc{Additionally, in \S\ref{cpsec} we give an outlook on case 
(d) $c_0=0.75$, 
from Fig.\ref{neigs}, where $\CC_L$ is unstable for all $\Lam$.}

In the numerics we (as always) have to find a compromise between 
speed and accuracy. For the default $L=10$ we start with an initial 
discretization of the straight cylinder $\CC_L$ by $n_p\approx 3000$ 
mesh points; the continuation of the nontrivial branches then often 
requires mesh refinement (and coarsening), typically leading 
to meshes of 4000 to 5000 points. For the longer cylinders for $c_0=0.48$ 
we increase this to up to 12000 mesh points. A simple measure of numerical 
resolution is the comparison of the $\lam_2$ values of the 
numerical BPs from $\CC_L$ with their analytical values from \S\ref{lineig}, 
and here we note that in all cases we have agreement of at least 4 digits. 
Moreover, we also compare 
some numerical nontrivial branches with their descriptions by the AEs, 
and find excellent agreement. 

\brem\label{vrem}{\rm 
Some cylindrical solutions have similarities with 
axisymmetric closed vesicle solutions of \reff{helf0}. 
We recall from \cite{JSL93} or \cite{geompap}, that from the sphere 
the first bifurcation is to  prolates (rods) and oblates 
(wafers). 
For mildly negative or positive $c_0$  the prolates are stable near 
bifurcation and the oblates unstable, and continuing the prolates 
they become dumbbells (two balls connected by a  neck), 
from which pea shaped vesicles bifurcate which become stable as one of the 
ball shrinks. For sufficiently 
negative $c_0$, the oblates are stable near bifurcation, and continuing 
the branch they become discocytes of biconcave red blood cell shape. 
Here we see some reminiscent behavior: For sufficiently negative $c_0$ 
we find secondary bifurcations of stable wrinkles with 
``embedded biconcave shapes'', see, e.g., Fig.\ref{cmf1}E. 
For sufficiently positive $c_0$, the primary pearling bifurcation 
leads to ``strings of dumbbells'' rather than strings of (round) pearls, 
see, e.g., samples C in Figures \ref{c05f1} and \ref{c05f1l}, or the 
samples A$_1$--A$_3$ in Fig.\ref{c1f1}. 
}\eex\erem 



We complement our results by some (area and volume conserving) 
numerical flows close to steady states, and for these 
perturb steady states $X_0$ in two different ways: one is 
%either in the form 
\huga{\label{flp1}
\tilde{X}_0=X_0+\del u_0N_0,\quad u_0=\frac 1{1+\xi x^2}\cos(\bphi), 
}
where $x$ is the coordinate along 
the cylinder axis, and $\bphi$ the polar angle orthogonal to it, 
and $\del\in\R$ and $\xi>0$ are parameters, with typically $\xi=1$ and 
$\del=-0.125$ or $\del=-0.25$ (recall that $N$ is the inner normal).  
The other way is  
\huga{\label{flp2}
\tilde{X}_0=X_0+\del u_0N_0,\quad 
\quad \text{with $u_0=\psi_{\text{crit}}$}, 
}
where $\psi_{\text{crit}}$ is 
(the $u$ component of) the eigenvector to the largest 
eigenvalue of the Jacobian 
at $X_0$, and typically $\del=-0.5$. 
Due to the negative $\del$ combined with the 
inner normal $N$, perturbations of type \reff{flp1} 
in general induce a small increase of the initial volume 
$\CV_0=\CV+\CV_\del$ and area $\CA_0=\CA+\CA_\del$, which are conserved 
under the flow. 
On the other hand, perturbations of type \reff{flp2} are 
area and volume preserving to linear order.  


Our numerical flows 
$t\mapsto (X(t),\Lam(t))=\Psinum(t;h)X_0$ are
{\em ad hoc} approximations  with a time stepsize $h$ 
and tolerance {\tt tol} (see Appendix \ref{num}), and  
we summarize the results from our flow experiments as follows:
\bcen 
\item Linearly stable $X_0$ (at $(\CV,\CA)$) are also stable under the flow 
at the perturbed $(\CV_0,\CA_0)$, and the solution flows back to the respective 
type (pearling, coiling, ...) at $(\CV_0,\CA_0)$, with a small 
change in $(\lam_1,\lam_2)$. See, e.g., Fig.\ref{c0f2}(a,b). 
\item If $X_0$ at $(\CV,\CA)$ is linearly unstable, then we generally 
expect $X(t)$ to flow to the nearest stable steady state 
(of in general a different class), see Fig.\ref{c0f2}(c$_2$). 
However, if we have a significant 
perturbation of $(\CA_0,\CV_0)$, then $X(t)$ may still flow to a similar 
steady state close to $X_0$ by adapting 
$(\lam_1,\lam_2)$, see, e.g., Fig.\ref{c0f2}($c_1$). 
This underlines the fact 
that $\lam_{1,2}$ are dynamical variables. 
\item Naturally, we want $E$ to decrease monotonously in $t$, cf.\reff{helf1b}, 
which if violated gives an easy indicator of poor numerics. 
The monotonous decrease of $E$ often requires rather small stepsizes 
and tolerances, and a result is that in many examples 
a single numerical flow to steady state is as expensive as 
the computation of the full BD of steady states, 
which we take as a strong argument 
for our steady state continuation and bifurcation approach. 
\item \huc{For $c_0=0.75$, where $\CC_L$ is always unstable and hence 
no stable primary bifurcations occur, we can numerically flow 
to stable finite wavelength pearling, which we subsequently continue in 
parameters, see Fig.\ref{c1f1}. However, this is only an outlook, 
and we leave a detailed and systematic study of this for future work.}
\ecen 

%\input{c0f1}

\subsection{$c_0=0$}
For $L=10$ and $c_0=0$, \S\ref{stabrange} gives that the cylinder 
destabilizes at $\lam_2\approx -0.95$ to pearling $(k_1,0)$, 
and at $\lam_2\approx 1.19$ to coiling/buckling $(k_1,1)$. 
Figure \ref{c00f} shows the BDs and samples starting in 
(a$_1$) with the energy $E$ over the reduced volume $v$.  
\input{c0f1}
Here all branches 
bifurcate from $v=1$, but (a$_2$) shows that they are well separated in 
the $(\lam_1,\lam_2)$ plane. 
As stated in \autoref{pea-stab}, the blue pearling branch starts stable 
close to the bifurcation point (sample A$_1$), and stays stable up 
to rather strong deformations of the original cylinder, sample A$_2$. 
The area constraint prevents the branch from growing to arbitrary volumes, 
but due to neck development the continuation becomes more difficult for 
larger $v$. 
From the mode $(m,n)=(1,1)$ at $\lam_2\approx 1.19$ we find 
buckling and coiling. The coefficients in \reff{ampsys} 
are $(a,b_1,b_2)=(0.39,-0.4,-0.67)$, 
 and as predicted (see Remark \ref{arem1}) 
the coiling (sample B) is stable close to bifurcation, 
while the buckling (sample C) is unstable. This 
behavior continues to small $v$, with no secondary bifurcations. 

Additionally we show one wrinkling %(non--axisymmetric but homogeneous in $x$) 
branch (sample D) as a  later bifurcation from the cylinder, and 
a secondary bifurcation to a wrinkling--buckling mix (sample E). 
However, these solutions are all linearly unstable in the $\lam_{1,2}$ range 
shown, at the given $\CV$ and $\CA$. 

%\input{c0f1}

\input{ampcomf1}

\brem\label{arem1} 
The amplitude formalism in \autoref{redeq} is only expected 
to be valid in a small neighborhood of the bifurcation points.  
In Fig.~\ref{ampc00f} we show comparisons between the numerical 
computations and the AE predictions. 
Here the amplitude formalism 
for the pearling
\hugast{ 
\text{$u=\eps A\psi_{10}+\CO(\eps^2)$,\quad $\lam_2=\lam_2(1,0)-\eps^2$, 
\quad $\lam_1=\lam_1(1,0)+\al_2\eps^2+\CO(\eps^4)$,}
}  
yields $\ds \ddT A =A(0.61-2.96A^2)$ and $\al_2= 0.66 A^2-1$, 
%\hueqst{\ddT A =A(-2.96A^2+0.61), \lam_2=\lam_2(1,0)-\eps^2\quad \al_2= 0.66 A^2-1, } 
and that for the wrinkling $u=\eps A\psi_{01}+\CO(\eps^2)$, 
$\lam_2=\lam_2(0,1)+\eps^2$, $\lam_1=\lam_1(0,1){+}\al_2\eps^2{+}\CO(\eps^4)$
yields the universal AE \reff{wria1}, i.e., 
$\ds \ddT A=A(3{-}15.19A^2)$ and $\al_2=\frac {27} 2 A^2{-}1$. 
For both, pearling and wrinkling,  we find an excellent match with the numerics. 
\eex\erem

%\input{ampcomf1}



In Fig.\ref{c0f2} we show numerical flows from the steady states A--C 
from Fig.\ref{c00f}, perturbed according to \reff{flp1}, with parameters 
given in Table \ref{ptab1}. In all cases we integrate until %$t\ge 0.5$ and 
$\|\pa_t u\|_\infty<0.001$. The plots on the left show the initially perturbed 
$X_0$, and $X$ at the end of the DNS colored by the last update $\del u$, 
such that $u_t\approx \del u/h$, where $h$ is the current stepsize. 
The plots on the right show the evolution of $E(t)$ and $\lam_{1,2}$, 
and the relative errors in $\CA$ and $\CV$ (with the error in $\CV$ 
always two orders of magnitude larger than that in $\CA$). 

\input{c0f2}


The first two flows start near stable steady 
states $(X_0,\lam_{1,0},\lam_{2,0})$, and as expected flow back to 
near $X_0$ rather quickly, with partly significant 
changes of $(\lam_1,\lam_2)$. 
However, the third flow (c$_1$) is somewhat surprising. 
State C from Fig.\ref{c00f} 
is linearly unstable, but the perturbed $X_0$ flows to another 
buckling by adjusting $\lam_{1,2}$ at the increased area and 
volume, where this buckling is stable. On the other hand, in (c$_2$) 
for the 
(linearly) area and volume preserving initial perturbation into the 
most unstable direction (which point towards coiling), 
the behavior is different: The solution now converges to coiling, 
with a rather small flow throughout; 
$\lam_1$ hardly changes at all, $\lam_2$ only very slightly, 
and the convergence is very slow (since the leading eigenvalue 
of the target coiling is negative but very close to zero). For all flows, we can use 
the final state as an initial guess for steady state 
continuation (e.g., in $\lam_2$), 
and the obtained numerical steady states then are (volume preserving) 
linearly stable. 

\input{ftab1}

\input{cmf1a}
\subsection{$c_0=-1$}
For (strongly) negative $c_0$, the wrinkling branches and their secondary  
bifurcations
become relevant. Fig.\ref{cmf1} shows basic results 
for $c_0{=}-1$ and $L{=}10$. 
As before, at negative $\lam_2\approx -2.254$ 
and $\lam_1\approx 1.5$ (cf.Fig.\ref{neigs}), $\Cr$ loses stability 
to pearling, but now at positive $\lam_2=3/2$ and $\lam_1=-9/4$ 
it loses stability to the wrinkling branch (samples D$_{1,2}$), while the 
bifurcation to buckling and coiling is at a later $(\lam_1,\lam_2)\approx 
(-3.77,3.021)$ and yields initially unstable branches. 
The wrinkling is initially stable, but 
at $\lam_2\approx 1.6$ loses stability to ``oblates embedded in wrinkling'', 
see sample E, and Remark \ref{vrem}. 
%\input{cmf1b}

Figure \ref{cmf2} shows some numerical flows from states from Fig.\ref{cmf1}, 
focusing on wrinkling perturbed according to \reff{flp1} 
(pearling is again stable, also under rather large perturbations). 
D$_2$ at its given $(\CA_0,\CV_0)$ is linearly (weakly) unstable, 
and the perturbation yields a slow evolution to an oblate wrinkling, 
with a very small change in $E$. In (b) and (c) we perturb a coiling and 
a buckling, and in both cases flow to wrinkling, and the bottom 
line of Fig.\ref{cmf2} and similar 
experiments is that (stable) wrinkling and oblate wrinkling 
have rather large domains of attraction. 
For completeness, Fig.\ref{cmf1b} shows a comparison with 
the AE predictions from \reff{wria1} for wrinkling, again with very good 
agreement, cf.~Remark \ref{arem1}. 

%\input{cmf1}

\input{cmf2}

\input{cmf1b}

%\clearpage
\subsection{$c_0=0.48$}
\huc{We now consider 
$c_0\in(1/4,1/2)$}, specifically $c_0=0.48$, cf.~Fig.\ref{neigs}(c). 
By Corollary \ref{destabcor}, 
the cylinder destabilizes in a {\em finite wavelength} pearling instability, 
and in a long wave instability to coiling and 
buckling. The finite pearling period is $\ell:=\ell_p\approx 7.5$, and thus 
we will be mostly interested in length $L$ as multiples of $7.5$. 

However, for comparison with the cases $c_0=0$ and $c_0=-1$ 
we first again choose $L=10$, and in Fig.\ref{c005f2} give the BD of buckling 
and coiling. The coefficients for the AE description \reff{ampsys} now 
are $(a,b_1,b_2)=(0.39,-0.083, 0.56)$, and in agreement with Fig.\ref{stabfig} 
the buckling is now stable at bifurcation and the coiling is unstable. 
Moreover, we find interesting secondary bifurcations on both branches, 
where the buckling loses (coiling gains) stability, and these two BPs 
are connected by a stable intermediate branch, see sample C. The comparison 
with the AEs in (c) again shows the agreement close to bifurcation, but 
naturally the (cubic order) AEs cannot capture the fold of the coiling  
in $\lam_2$. 

\input{c0048f2}

\input{c05f1c}


Figure \ref{c05f1} shows the BD and samples for $L{=}15$. 
To the right of $v{=}1$ bifurcates the $k_2{\approx}0.838$ pearling branch 
(at $\lam_2{\approx}-0.243$), and 
is initially stable (sample A$_1$). However, shortly after 
($\lam_2{\approx}-0.3756$) there 
is a secondary bifurcation to a stable branch with double the period, 
sample B. 
On the other hand, the primary $m{=}1$ pearling branch, sample C, 
(bifurcating at $\lam_2{\approx}-0.421$) is unstable throughout.%
\footnote{\huc{At first sight, C may look similar to the $m=2$ pearling A$_1$ and 
A$_2$, but the difference is that C has one weak and one stronger constriction, 
which intuitely makes C one period in a string of dumbbells; 
see also C in Fig.~\ref{c05f1l}, and Remark \ref{vrem}.}}
The $(m,n){=}(1,1)$ coiling (sample D) and buckling (sample E) 
bifurcate at $\lam_2{\approx}0.138$, 
and again the coiling is stable, and stays stable to rather small $v$, 
while the buckling is unstable. Wrinkling does not occur in the 
parameter regime considered; however, the 
(compared to $L=10$ before) slightly larger $L=15$  
lets the pearling and coiling/buckling BPs move closer together, which is 
why we chose 
to also present the $(m,n)=(2,1)$ coiling F (unstable). 
Figure \ref{c05f2} shows the flow from a perturbation of A$_2$ to a B 
type solution but rather close to the BP. 
Therefore, the convergence to steady state is again very slow, as 
near bifurcation the stable B branch has a leading eigenvalue close to $0$. 

%\input{c05f1c}

\input{c05f1c2}

\input{c05f1l}

The main point of Fig.\ref{c05f1} is that the choice of $c_0=0.48$ 
together with $L=15$ yields the destabilization 
of the cylinder to the $k_2\approx 0.838$ pearling, but these solutions are only 
stable in a somewhat narrow range (in $v$, say). To further assess this, 
in Fig.\ref{c05f1l} we consider the primary pearling with $\ell=7.5$ 
on twice the domain $L=30$. 
The result shows that the range  of stable $\ell=7.5$ pearling 
shrinks with increasing $L$, and this continues for further increase of 
$L$, 
yielding the following dependence of the reduced volume $v_s$ of single 
pearling BPs from primary $\ell=7.5$ pearling on $L$: 
\huga{\label{ptt1}
\begin{tabular}{c|cccc}
$L$&15&39&45&60\\
$v_s$&1.0081&1.0063&1.0046&1.0035
\end{tabular}
}
We also ran some numerical flows from 
perturbations of A in Fig.\ref{c05f1l}, and similarly at larger $L$, 
with results as in Fig.\ref{c05f2}, i.e., convergence to the 
single pearling solutions. However, these DNS are very expensive, 
partly due to the larger domain and hence larger scale discretization, 
but more importantly due to the very slow convergence of the flows.  

%\input{c05f1l}

%\input{c075}

%\input{c1f1}
\subsection{Outlook: $c_0=0.75$}\label{cpsec}
Lastly, following Fig.\ref{neigs}(e) we consider 
$c_0>1/2$, specifically $c_0=0.75$ for which 
$\CC_L$ is never stable if $L\ge 2\pi $ ($k_1\le 1$, say), and    
branches as before still bifurcate from $\CC_L$, 
but not at loss of stability of $\CC_L$. 
Hence they can also still be described by AEs as before, but they cannot 
be stable close to bifurcation, and we can only expect stable ``patterns'' 
at $O(1)$ amplitude. This is more difficult than 
the analysis and numerics so far, and hence here we only give 
an outlook on some interesting (numerical) results we obtain, 
again for a rather small length $L=10$ of the cylinder, and 
leave more systematic and detailed studies to later work. 

\input{c1f1}

Figure \ref{c1f1} shows the BD of $k_1\approx 0.628$ pearling 
(A, blue) and $k_2\approx 1.257$ pearling (C, light blue), 
which are both unstable at bifurcation as they must, and 
moreover are unstable throughout, 
and addtionally an $O(1)$ amplitude pearling branch (P, red), 
where P$_2$ is obtained from DNS  starting 
near A$_1$ (panel (c)). In summary, we see a number of new effects which 
strongly suggest further study, but here we restrict to the following comments.

$\bullet$ We stop the continuations shortly after A$_3$, shortly 
after C, and shortly after P$_1$ as further continuations there 
require excessive mesh adaptations. We can continue significantly 
beyond P$_3$, but our main region of interest is near $v=1$. 
There are bifurcations on the blue branches which break the 
rotational symmetry, but we restrict to presenting axisymmetric branches. 

$\bullet$ The $k_1$ pearling branch A shows two folds in $v$, 
the first at $v_{f,1}\approx 1.045$, the second at 
$v_{f,2}\approx 0.98$. In particular, between A$_1$ and A$_2$ 
it goes through $v=1$ again, while keeping the area $\CA$ 
constant throughout. This is not a contradiction to the fact 
that normal variations of $\CC_L$ that fix $\CA$ and $\CV$ 
locally do not exist; the passage through $v=1$ here 
corresponds to a non--small normal variation. 

$\bullet$ The folds on the 
A branch naturally call for fold continuation in $c_0$, in 
particular for decreasing $c_0$ as for $c_0<1/2$ we do not see 
folds on the analogous A branches. We believe that they vanish 
at some $c_0>1/2$ as the blue swallowtail shrinks and the folds 
collide, but this remains to be studied. 
%Presently we can only do this in a very inefficient way largely based on numerical Jacobians for the extended system for the fold continuation, and this needs to be improved first. The same applies to branch point continuation as another relevant two--parameter problem. 

$\bullet$ The flow in (c) starts at A$_1$ with a small pertubation 
in direction of the most unstable eigenvalue; 
A$_1$ is below the fold, and there is exactly one 
positive eigenvalue $\mu\approx 0.2$. In any case, 
the results of flow experiments seem rather robust wrt 
the choice of the initial conditions (choice of steady state 
and perturbation), i.e., we always ``land'' on the P branch, 
though naturally at different $v$ and $\lam_2$, or analoga 
of the P branch at different area $\CA$. In the particular 
case shown, the perturbation of A$_1$ yields a relative 
change of $\CV$ of order $10^{-3}$, and a relative change of 
$\CA$ of order $10^{-4}$. (The initial perturbation 
{\em linearly} conserves $\CA$ and $\CV$, i.e., 
is tangential to the constraint manifold, but 
for any finite perturbation we must expect a (nonlinear) 
change of $\CA$ and $\CV$. However, the change in $\CA$ is 
so small that we ignore it and keep the normalization of 
$E$ in \reff{enorm} by the original $\CA$.) 

$\bullet$ The last plots in (c) suggest almost steady states for $t>20$, 
and we use the solution at $t=20.95$ as an initial guess for 
Newton's method for the steady problem. This indeed takes us to the 
(spectrally) stable steady state P$_2$, and continuing 
from here to larger/smaller $v$ yields the red branch. 

$\bullet$ It is remarkable that the P branch with two pearls of different 
sizes  is stable, that along the branch the pearls change their relative 
sizes (different from the primary pearling branches, where only 
the global amplitude changes), 
and that in fact P$_2$ attracts (perturbations of) A$_1$.  
However, some finite size effects are involved here, because some stability 
of the P branch is lost when 
repeating the experiment from Fig.\ref{c1f1} on larger domains, 
e.g., $L=20$. In this case, initial conditions for numerical flows 
must be chosen more carefully, namely closer to $v=1$ to reach the analogue 
of the P branch (4 pearls on $L=20$), and continuation of the P branch 
then shows a loss of stability (wrt to still axially symmetric solutions) 
away from $v=1$. 
We plan to study in particular these effects 
in a systematic way in future work, including their relation 
to the transition from A to B in Fig.~\ref{c05f1l}. %\hfill\mbox{{}}

$\bullet$ Shape wise (compare P$_1$ and C in (d)) it seems possible 
that the P branch connects to the C branch in a period--doubling 
bifurcation, but samples  P$_1$ and C are at rather different values of 
$\lam_{1,2}$. In our preliminary experiments so far we could not 
identify to what  other branches the P branch connects, and again we 
leave this for future work. 



%\input{c1f1}


  




==> numexb1.tex <==
\section{Numerical examples} \label{numex}
We now use numerical continuation and bifurcation methods 
to corroborate the local results from 
\S\ref{aesec}, and to extend them to a more global picture. 
This includes some secondary bifurcations with interesting stable 
shapes away from the straight cylinder. The numerical setup follows 
the stability analysis in \autoref{stabrange} and \S\ref{redeq}. 
Namely, we fix a period $L$ (e.g., $L=10$, $L=15$ or $L=30$, see 
also Remark \ref{carem}),  and the area $\CA=\CA(X)$, and 
initially use $\lam_2$ as the primary bifurcation parameter 
and $\lam_1$ and $\CV(X)$ as secondary (dependent) parameters. 
The linearized stability of the solutions, however, is then computed for 
fixed $\CA(X)$ and $\CV(X)$ while $\lam_1$ and $\lam_2$ are free parameters. 
Due to the radius-length scaling invariance of the Helfrich energy \reff{helfen} and the area and volume constraint in the dynamical 
problem, it is useful to introduce the reduced volume  
\hueq{\label{redvol} v=\CV(X)/\CV_0,} 
 where $\CV_0$ is the volume of the straight cylinder with the same $\CA(X)$, 
compare \cite{JSL93}, and we normalize the energy 
\hueq{\label{enorm}
\tilde E(X)=\frac 1 \CA \int_X (H-c_0)^2\dd S.} 
Also for our numerics we focus on the three exemplary cases 
\hugast{
\text{(a) $c_0=0$,\quad (b) $c_0=-1$, \quad and (c) $c_0=0.48$}
} 
from Fig.\ref{neigs}, and mostly 
we use $L=10$. For (a) and (b) 
this is no significant restriction as in these cases the primary 
bifurcations (to pearling, buckling and coiling in (a), and to pearling and 
wrinkling in (b)) are of long wave type for any (sufficiently large) $L$, 
i.e., a different $L$ gives the same types of primary bifurcations with 
different axial (maximal) periods $L$ (and the wrinkling is independent of $L$). 
However, for (c) and sufficiently large $L$ (preferably an integer 
multiple of the critical period $\ell\approx 7.5$) we have a 
finite wave number pearling instability. Thus, besides the case $L{=}10$ 
(for comparison with (a) and (b)), for (c) we shall consider different 
multiples of 7.5 for $L$, namely $L{=}15, L{=}30$, and $L{=}45$, allowing 
2, 4, and 6, pearls on the primary branch. The influence of $L$ 
will then be the behavior of this branch away from bifurcation, 
which loses stability in a bifurcation to a single pearl branch, 
and this BP moves closer to the primary BP with increasing $L$. 
This is further discussed in \S\ref{dsec}. 
\huc{Additionally, in \S\ref{cpsec} we give an outlook on case 
(d) $c_0=0.75$, 
from Fig.\ref{neigs}, where $\CC_L$ is unstable for all $\Lam$.}

In the numerics we (as always) have to find a compromise between 
speed and accuracy. For the default $L=10$ we start with an initial 
discretization of the straight cylinder $\CC_L$ by $n_p\approx 3000$ 
mesh points; the continuation of the nontrivial branches then often 
requires mesh refinement (and coarsening), typically leading 
to meshes of 4000 to 5000 points. For the longer cylinders for $c_0=0.48$ 
we increase this to up to 12000 mesh points. A simple measure of numerical 
resolution is the comparison of the $\lam_2$ values of the 
numerical BPs from $\CC_L$ with their analytical values from \S\ref{lineig}, 
and here we note that in all cases we have agreement of at least 4 digits. 
Moreover, we also compare 
some numerical nontrivial branches with their descriptions by the AEs, 
and find excellent agreement. 

\brem\label{vrem}{\rm 
Some cylindrical solutions have similarities with 
axisymmetric closed vesicle solutions of \reff{helf0}. 
We recall from \cite{JSL93} or \cite{geompap}, that from the sphere 
the first bifurcation is to  prolates (rods) and oblates 
(wafers). 
For mildly negative or positive $c_0$  the prolates are stable near 
bifurcation and the oblates unstable, and continuing the prolates 
they become dumbbells (two balls connected by a  neck), 
from which pea shaped vesicles bifurcate which become stable as one of the 
ball shrinks. For sufficiently 
negative $c_0$, the oblates are stable near bifurcation, and continuing 
the branch they become discocytes of biconcave red blood cell shape. 
Here we see some reminiscent behavior: For sufficiently negative $c_0$ 
we find secondary bifurcations of stable wrinkles with 
``embedded biconcave shapes'', see, e.g., Fig.\ref{cmf1}E. 
For sufficiently positive $c_0$, the primary pearling bifurcation 
leads to ``strings of dumbbells'' rather than strings of (round) pearls, 
see, e.g., samples C in Figures \ref{c05f1} and \ref{c05f1l}), or the 
samples A$_1$--A$_3$ in Fig.\ref{c1f1}. 
}\eex\erem 



We complement our results by some (area and volume conserving) 
numerical flows close to steady states, and for these 
perturb steady states $X_0$ in two different ways: one is 
%either in the form 
\huga{\label{flp1}
\tilde{X}_0=X_0+\del u_0N_0,\quad u_0=\frac 1{1+\xi x^2}\cos(\bphi), 
}
where $x$ is the coordinate along 
the cylinder axis, and $\bphi$ the polar angle orthogonal to it, 
and $\del\in\R$ and $\xi>0$ are parameters, with typically $\xi=1$ and 
$\del=-0.125$ or $\del=-0.25$ (recall that $N$ is the inner normal).  
The other way is  
\huga{\label{flp2}
\tilde{X}_0=X_0+\del u_0N_0,\quad 
\quad \text{with $u_0=\psi_{\text{crit}}$}, 
}
where $\psi_{\text{crit}}$ is 
(the $u$ component of) the eigenvector to the largest 
eigenvalue of the Jacobian 
at $X_0$, and typically $\del=-0.5$. 
Due to the negative $\del$ combined with the 
inner normal $N$, perturbations of type \reff{flp1} 
in general induce a small increase of the initial volume 
$\CV_0=\CV+\CV_\del$ and area $\CA_0=\CA+\CA_\del$, which are conserved 
under the flow. 
On the other hand, perturbations of type \reff{flp2} are 
area and volume preserving to linear order.  


Our numerical flows 
$t\mapsto (X(t),\Lam(t))=\Psinum(t;h)X_0$ are
{\em ad hoc} approximations  with a time stepsize $h$ 
and tolerance {\tt tol} (see Appendix \ref{num}), and  
we summarize the results from our flow experiments as follows:
\bcen 
\item Linearly stable $X_0$ (at $(\CV,\CA)$) are also stable under the flow 
at the perturbed $(\CV_0,\CA_0)$, and the solution flows back to the respective 
type (pearling, coiling, ...) at $(\CV_0,\CA_0)$, with a small 
change in $(\lam_1,\lam_2)$. See, e.g., Fig.\ref{c0f2}(a,b). 
\item If $X_0$ at $(\CV,\CA)$ is linearly unstable, then we generally 
expect $X(t)$ to flow to the nearest stable steady state 
(of in general a different class), see Fig.\ref{c0f2}(c$_2$). 
However, if we have a significant 
perturbation of $(\CA_0,\CV_0)$, then $X(t)$ may still flow to a similar 
steady state close to $X_0$ by adapting 
$(\lam_1,\lam_2)$, see, e.g., Fig.\ref{c0f2}($c_1$). 
This underlines the fact 
that $\lam_{1,2}$ are dynamical variables. 
\item Naturally, we want $E$ to decrease monotonously in $t$, cf.\reff{helf1b}, 
which if violated gives an easy indicator of poor numerics. 
The monotonous decrease of $E$ often requires rather small stepsizes 
and tolerances, and a result is that in many examples 
a single numerical flow to steady state is as expensive as 
the computation of the full BD of steady states, 
which we take as a strong argument 
for our steady state continuation and bifurcation approach. 
\item \huc{For $c_0=0.75$, where $\CC_L$ is always unstable and hence 
no stable primary bifurcations occur, we can numerically flow 
to stable finite wavelength pearling, which we subsequently continue in 
parameters, see Fig.\ref{c1f1}. However, this is only an outlook, 
and we leave a detailed and systematic study of this for future work.}
\ecen 

%\input{c0f1}

\subsection{$c_0=0$}
For $L=10$ and $c_0=0$, \S\ref{stabrange} gives that the cylinder 
destabilizes at $\lam_2\approx -0.95$ to pearling $(k_1,0)$, 
and at $\lam_2\approx 1.19$ to coiling/buckling $(k_1,1)$. 
Figure \ref{c00f} shows the BDs and samples starting in 
(a$_1$) with the energy $E$ over the reduced volume $v$.  
\input{c0f1}
Here all branches 
bifurcate from $v=1$, but (a$_2$) shows that they are well separated in 
the $(\lam_1,\lam_2)$ plane. 
As stated in \autoref{pea-stab}, the blue pearling branch starts stable 
close to the bifurcation point (sample A$_1$), and stays stable up 
to rather strong deformations of the original cylinder, sample A$_2$. 
The area constraint prevents the branch from growing to arbitrary volumes, 
but due to neck development the continuation becomes more difficult for 
larger $v$. 
From the mode $(m,n)=(1,1)$ at $\lam_2\approx 1.19$ we find 
buckling and coiling. The coefficients in \reff{ampsys} 
are $(a,b_1,b_2)=(0.39,-0.4,-0.67)$, 
 and as predicted (see Remark \ref{arem1}) 
the coiling (sample B) is stable close to bifurcation, 
while the buckling (sample C) is unstable. This 
behavior continues to small $v$, with no secondary bifurcations. 

Additionally we show one wrinkling %(non--axisymmetric but homogeneous in $x$) 
branch (sample D) as a  later bifurcation from the cylinder, and 
a secondary bifurcation to a wrinkling--buckling mix (sample E). 
However, these solutions are all linearly unstable in the $\lam_{1,2}$ range 
shown, at the given $\CV$ and $\CA$. 

%\input{c0f1}

\input{ampcomf1}

\brem\label{arem1} 
The amplitude formalism in \autoref{redeq} is only expected 
to be valid in a small neighborhood of the bifurcation points.  
In Fig.~\ref{ampc00f} we show comparisons between the numerical 
computations and the AE predictions. 
Here the amplitude formalism 
for the pearling
\hugast{ 
\text{$u=\eps A\psi_{10}+\CO(\eps^2)$,\quad $\lam_2=\lam_2(1,0)-\eps^2$, 
\quad $\lam_1=\lam_1(1,0)+\al_2\eps^2+\CO(\eps^4)$,}
}  
yields $\ds \ddT A =A(0.61-2.96A^2)$ and $\al_2= 0.66 A^2-1$, 
%\hueqst{\ddT A =A(-2.96A^2+0.61), \lam_2=\lam_2(1,0)-\eps^2\quad \al_2= 0.66 A^2-1, } 
and that for the wrinkling $u=\eps A\psi_{01}+\CO(\eps^2)$, 
$\lam_2=\lam_2(0,1)+\eps^2$, $\lam_1=\lam_1(0,1){+}\al_2\eps^2{+}\CO(\eps^4)$
yields the universal AE \reff{wria1}, i.e., 
$\ds \ddT A=A(3{-}15.19A^2)$ and $\al_2=\frac {27} 2 A^2{-}1$. 
For both, pearling and wrinkling,  we find an excellent match with the numerics. 
\eex\erem

%\input{ampcomf1}



In Fig.\ref{c0f2} we show numerical flows from the steady states A--C 
from Fig.\ref{c00f}, perturbed according to \reff{flp1}, with parameters 
given in Table \ref{ptab1}. In all cases we integrate until %$t\ge 0.5$ and 
$\|\pa_t u\|_\infty<0.001$. The plots on the left show the initially perturbed 
$X_0$, and $X$ at the end of the DNS colored by the last update $\del u$, 
such that $u_t\approx \del u/h$, where $h$ is the current stepsize. 
The plots on the right show the evolution of $E(t)$ and $\lam_{1,2}$, 
and the relative errors in $\CA$ and $\CV$ (with the error in $\CV$ 
always two orders of magnitude larger than that in $\CA$). 

\input{c0f2}


The first two flows start near stable steady 
states $(X_0,\lam_{1,0},\lam_{2,0})$, and as expected flow back to 
near $X_0$ rather quickly, with partly significant 
changes of $(\lam_1,\lam_2)$. 
However, the third flow (c$_1$) is somewhat surprising. 
State C from Fig.\ref{c00f} 
is linearly unstable, but the perturbed $X_0$ flows to another 
buckling by adjusting $\lam_{1,2}$ at the increased area and 
volume, where this buckling is stable. On the other hand, in (c$_2$) 
for the 
(linearly) area and volume preserving initial perturbation into the 
most unstable direction (which point towards coiling), 
the behavior is different: The solution now converges to coiling, 
with a rather small flow throughout; 
$\lam_1$ hardly changes at all, $\lam_2$ only very slightly, 
and the convergence is very slow (since the leading eigenvalue 
of the target coiling is negative but very close to zero). For all flows, we can use 
the final state as an initial guess for steady state 
continuation (e.g., in $\lam_2$), 
and the obtained numerical steady states then are (volume preserving) 
linearly stable. 

\input{ftab1}

\input{cmf1a}
\subsection{$c_0=-1$}
For (strongly) negative $c_0$, the wrinkling branches and their secondary  
bifurcations
become relevant. Fig.\ref{cmf1}(a,b) shows basic results 
for $c_0{=}-1$ and $L{=}10$, and (c) a comparison with 
the AE predictions from \reff{wria1} for wrinkling, again with very good 
agreement, cf.~Remark \ref{arem1}. 
As before, at negative $\lam_2\approx -2.254$ 
and $\lam_1\approx 1.5$ (cf.Fig.\ref{neigs}), $\Cr$ loses stability 
to pearling, but now at positive $\lam_2=3/2$ and $\lam_1=-9/4$ 
it loses stability to the wrinkling branch (samples D$_{1,2}$), while the 
bifurcation to buckling and coiling is at a later $(\lam_1,\lam_2)\approx 
(-3.77,3.021)$ and yields initially unstable branches. 
The wrinkling is initially stable, but 
at $\lam_2\approx 1.6$ loses stability to ``oblates embedded in wrinkling'', 
see sample E, and Remark \ref{vrem}. 
%\input{cmf1a}

Figure \ref{cmf2} shows some numerical flows from states from Fig.\ref{cmf1}, 
focusing on wrinkling perturbed according to \reff{flp1} 
(pearling is again stable, also under rather large perturbations). 
D$_2$ at its given $(\CA_0,\CV_0)$ is linearly (weakly) unstable, 
and the perturbation yields a slow evolution to an oblate wrinkling, 
with a very small change in $E$. In (b) and (c) we perturb a coiling and 
a buckling, and in both cases flow to wrinkling, and the bottom 
line of Fig.\ref{cmf2} and similar 
experiments is that (stable) wrinkling and oblate wrinkling 
have rather large domains of attraction. 

%\input{cmf1}

\input{cmf2}

%\clearpage
\subsection{$c_0=0.48$}
\huc{We now consider 
$c_0\in(1/4,1/2)$}, specifically $c_0=0.48$, cf.~Fig.\ref{neigs}(c). 
By Corollary \ref{destabcor}, 
the cylinder destabilizes in a {\em finite wavelength} pearling instability, 
and in a long wave instability to coiling and 
buckling. The finite pearling period is $\ell:=\ell_p\approx 7.5$, and thus 
we will be mostly interested in length $L$ as multiples of $7.5$. 

However, for comparison with the cases $c_0=0$ and $c_0=-1$ 
we first again choose $L=10$, and in Fig.\ref{c005f2} give the BD of buckling 
and coiling. The coefficients for the AE description \reff{ampsys} now 
are $(a,b_1,b_2)=(0.39,-0.083, 0.56)$, and in agreement with Fig.\ref{stabfig} 
the buckling is now stable at bifurcation and the coiling is unstable. 
Moreover, we find interesting secondary bifurcations on both branches, 
where the buckling loses (coiling gains) stability, and these two BPs 
are connected by a stable intermediate branch, see sample C. The comparison 
with the AEs in (c) again shows the agreement close to bifurcation, but 
naturally the (cubic order) AEs cannot capture the fold of the coiling  
in $\lam_2$. 

\input{c0048f2}

%\input{c05f1c}


Figure \ref{c05f1} shows the BD and samples for $L=15$. 
To the right of $v=1$ bifurcates the $k_2\approx 0.838$ pearling branch 
(at $\lam_2\approx -0.243$), and 
is initially stable (sample A$_1$). However, shortly after 
($\lam_2\approx -0.3756$) there 
is a secondary bifurcation to a stable branch with double the period, 
sample B. 
On the other hand, the primary $m=1$ pearling branch, sample C, 
(bifurcating at $\lam_2\approx -0.421$) is unstable throughout.%
\footnote{\huc{At first sight, C may look similar to the $m=2$ pearling A$_1$ and 
A$_2$, but the difference is that C has one small and one large constriction, 
which intuitely makes C one period in a string of dumbbells; 
see also C in Fig.~\ref{c05f1l}, and Remark \ref{vrem}.}}
The $(m,n)=(1,1)$ coiling (sample D) and buckling (sample E) 
bifurcate at $\lam_2\approx 0.138$, 
and again the coiling is stable, and stays stable to rather small $v$, 
while the buckling is unstable. Wrinkling does not occur in the 
parameter regime considered; however, the 
(compared to $L=10$ before) slightly larger $L=15$  
lets the pearling and coiling/buckling BPs move closer together, which is 
why we chose 
to also present the $(m,n)=(2,1)$ coiling F (unstable). 
Figure \ref{c05f2} shows the flow from a perturbation of A$_2$ to a B 
type solution but rather close to the BP. 
Therefore, the convergence to steady state is again very slow, as 
near bifurcation the stable B branch has a leading eigenvalue close to $0$. 

\input{c05f1c}

\input{c05f1c2}

The main point of Fig.\ref{c05f1} is that the choice of $c_0=0.48$ 
together with $L=15$ yields the destabilization 
of the cylinder to the $k_2\approx 0.838$ pearling, but these solutions are only 
stable in a somewhat narrow range (in $v$, say). To further assess this, 
in Fig.\ref{c05f1l} we consider the primary pearling with $\ell=7.5$ 
on twice the domain $L=30$. 
The result shows that the range  of stable $\ell=7.5$ pearling 
shrinks with increasing $L$, and this continues for further increase of 
$L$, 
yielding the following dependence of the reduced volume $v_s$ of single 
pearling BPs from primary $\ell=7.5$ pearling on $L$: 
\huga{\label{ptt1}
\begin{tabular}{c|cccc}
$L$&15&39&45&60\\
$v_s$&1.0081&1.0063&1.0046&1.0035
\end{tabular}
}
We also ran some numerical flows from 
perturbations of A in Fig.\ref{c05f1l}, and similarly at larger $L$, 
with results as in Fig.\ref{c05f2}, i.e., convergence to the 
single pearling solutions. However, these DNS are very expensive, 
partly due to the larger domain and hence larger scale discretization, 
but more importantly due to the very slow convergence of the flows.  

\input{c05f1l}

\input{c075}




==> stcyar.tex <==
\section{Stability of $\CC_L$}\label{stcy}
We consider the linearization of \reff{hflow} around $\CC_L(r)$. 
This requires some lengthy computations, but since $\CC_L(r)$ has 
constant mean and Gaussian curvatures (with $K=0$), we can explicitly 
compute the 
dispersion relation (Lemma \ref{leig}) and subsequently the stability ranges 
of and bifurcation points from $\CC_L(r)$ (Corollary \ref{destabcor}).
\subsection{Linearization and eigenvalues}\label{lineig}
Since $G(\cdot,\Lam):V^4_\eps\to L^2$ is an analytic map, 
we use \reff{meanu}, \reff{gaussu} and \reff{LBu} to calculate the 
Frech\'et derivative via the Gateaux differential in direction $v$, i.e., 
$\pa_u G(0,\Lam)v=\frac{\dd}{\dd \eps} G(\eps v,\Lam)|_{\eps=0}$; recall that  the Laplace-Beltrami operator on $\CC_L((r)$ is $\Delta_0=\pa_x^2+\frac 1 {r^2} \pa_\bphi^2$ in our coordinate system.
\blem \label{dcomp} The linearizations of 
$H(u), K(u)$, and $\Delta_uH(u)$ around $\CC_L(r)$, i.e., around $u=0$, 
are given by 
\hual{\label{dmean}\pa_u H(0)v&=-\frac 1 2\left(\Delta_0v +\frac 1 {r^2} v\right),\\
\label{dgauss}\pa_uK(0) v&=-r^{-1} \pa_x^2 v, \text{ and }\\[2mm]
\label{dlead}\pa_u \Delta_0H(0)v &= \Delta \pa_u H(0)v.
}
\elem

\begin{proof}
Using \reff{meanu} with $\eps v$ and sorting 
by $\eps$ powers gives
\hueqst{ 2H(\eps v)=-\frac{\eps(r^3 v_{xx}+rv_{\bphi\bphi}) +\CO(\eps^2)}{(r^2+\eps 2rv+\CO(\eps^2))^{3/2}}+\frac{1}{(r^2+\eps 2rv+\CO(\eps^2))^{1/2}}.}
Differentiating w.r.t. $\eps$ this gives 
\hueqst{\frac{\dd}{\dd \eps} 2 H(\eps v)=-\frac{(r^3 v_{xx}+rv_{\bphi\bphi})(r^2+\CO(\eps))^{3/2}+\CO(\eps)}{(r^2+\eps 2rv+\CO(\eps^2))^{3}}-\frac{r v+\CO(\eps)}{(r^2+\CO(\eps))^{3/2}}.}
The denominators are bounded away from zero, hence evaluating at $\eps=0$ gives \reff{dmean}.

For $K$ this works the same way, with 
\hueqst{ \frac{\dd}{\dd \eps} K(\eps v)= \frac{\dd}{\dd \eps}  \frac{-\eps r^3 v_{xx} +\CO(\eps^2)}{(r^2+2\eps 2rv+\CO(\eps^2))^2}=\frac{-r^3 v_{xx} ((r^2+\eps 2rv+O(\eps^2))^{2} +\CO(\eps)}{(r^2+\eps 2rv+\CO(\eps^2))^{4}}.}
Again evaluating at $\eps=0$ gives \reff{dgauss}. 

Finally for \reff{dlead} it is sufficient to notice that 
\hueqst{\frac{\dd}{\dd \eps} \Delta_{\eps v}H(\eps v)|_{\eps=0} 
= \left(\frac{\dd}{\dd \eps}\Delta_{\eps v} H(0)\right)\bigg|_{\eps=0} +\Delta_0  \left(\frac{\dd}{\dd \eps}H(\eps v)\bigg|_{\eps=0}\right)
=\Delta_0  \left(\frac{\dd}{\dd \eps}H(\eps v)\bigg|_{\eps=0}\right),}
since $H(0)$ is a constant and $\Delta_{\eps v}$ is non degenerate for small perturbations. 
\end{proof}

Inserting the expressions from Theorem \ref{dcomp} we obtain 
\blem $G(\cdot,\Lam)$ is Frechet differentiable at $u=0$, with differential, 
using \reff{socon}, 
\hual{\label{Gjac} \pa_uG(0,\Lam) v= -\frac 1 2\Delta^2_0 v-\left(r\lam_2+\frac{1}{r^2}\right) \Delta_0 v- \left(\frac{\lam_2}{r} +\frac{1}{2r^4}\right) v +\left(\frac 1 r-2c_0\right) r^{-1} \pa_x^2 v.
}
\elem
Over the unbounded $\CC(r)$, $\pa_uG(0,\Lam))$ has a continuous spectrum, 
but by restricting to the compact cylinder $\CC_L(r)$ of length $L$, 
 $\pa_uG(0,\Lam))$ has a discrete spectrum. 
%with a simple basis of eigenfunctions. 
\blem \label{leig}
The eigenvalue problem 
\hueq{ \label{eigeq}\pa_uG(0,\Lam)\psi=\mu\psi}
has a countable set of solutions $(\mu_{mn},\psi_{mn})\in 
\R\times H^4_{\per}(\CC_L(r))$,  $(m,n)\in\Z^2$, 
\bsub\label{eigs}
\hual{
&\text{$\psi_{mn}(x,\bphi)=e^{\ri (k_mx+n\bphi)}$, 
$k_m=2m\pi/L$, and $\mu_{mn}=\mu(k_m,n)$ with}\\
%\hual{\label{eigs} 
&\mu(k,n,\Lam)=-\frac 1 2  \Big[k^2{+}\frac {n^2} {r^2} \Big]^2 
+\left(r\lam_2{+}\frac{1}{r^2}\right)\Big[k^2{+}\frac {n^2} {r^2} \Big]
-\left(\frac{\lam_2}{r}{+}\frac{1}{2r^4}\right) 
-\left(\frac 1 r{-}2c_0\right) \frac{k^2}{r}.
}
\esub 
For all $\Lam\in\R^2$ the eigenfunctions $\psi_{0\pm1} \in\ker(\pa_uG(0,\Lam))$.
\elem
\begin{proof}
Recall that $H^4_{\per}(\CC_L(r))$ has a compact embedding in $L^2(\CC_L(r))$, 
hence the resolvent of \reff{Gjac} is compact. Using the $L^2$ basis of 
eigenfunctions of $\Delta_0$, 
\hueqst{ \psi_{mn}(x,\bphi)=e^{\ri(k_mx+n\bphi)}, \quad 
\Delta_0\psi_{mn}= -\Big[k_m^2+\frac 1 {r^2} n^2\Big]\psi_{mn}(x,\bphi), 
}
we obtain (\ref{eigs}b). 
Clearly $\mu(0,\pm1,\Lam)=0$, hence 
$\sin(\bphi),\cos(\bphi)\in \ker(\pa_uG(0,\Lam))$. 
\end{proof}

Using Lemma \ref{aderlem}, we write the linearization of \reff{hflowu} as 
\hual{ \label{genev0}\pa_U \sG(0,\Lam) U
& =\bpm \pa_u G(0,\Lam ) & \pa_{\lam_1} G(0,\Lam ) &\pa_{\lam_2} G(0,\Lam ) \\ 
		\pa_u \CA(0 ) & \pa_{\lam_1} \CA(0 ) &\pa_{\lam_2} \CA(0 )\\
		\pa_u \CV(0 ) & \pa_{\lam_1} \CV(0 ) &\pa_{\lam_2} \CV(0 )
		 \epm  \bpm u\\ \sig_1\\\sig_2\epm\nonumber\\
	&=\bpm \pa_u G(0,\Lam )u & -2H(0) \sig_1&-\sig_2 \\ 
		-\int_{\CC_L(r)} 2H(0) u\dd S &0 & 0\\
		\int_{\CC_L(r)} u \dd S& 0 & 0
\epm.}
The domain of $\pa_U\CG(0,\Lam)$ is $H^4_\per(\CC_L(r))\times \R^2$,  
equipped with the norm $\|U\|_{\pa_{(u,\Lam)}\sG}=\|u\|_{H^4}+\|\Sigma\|_{\R^2}$, and altogether we have the generalized eigenvalue problem 
\hual{ \label{genev}\pa_U \sG(0,\Lam) \Psi
= \mu \bpm 1 & 0& 0\\0 & 0& 0\\0 & 0& 0 \epm \Psi,\quad \Psi=(\psi,\sig_1,\sig_2),
}
with eigenvalues $\mu \in \{ \mu(k_m,n), \, (m,n)\in\Z^2\backslash \{(0,0)\}\cup \{0\}$ and eigenfunctions 
\hueqst{\Psi_{mn}= \bpm \psi_{mn}\\ 1\\ -2\epm, \, (m,n)\in\Z^2\backslash \{(0,0)\}, \text{ and }\Psi_{00}=\bpm 0\\ 1\\ -2\epm.
} 
\brem (a) The eigenvalues $\mu(0,\pm 1,\lam)=0$ correspond to 
translations of $\CC_L(r)$ in $y$ and $z$ directions. 
 Each eigenvalue of the form $\mu(k_m,0,\Lam)$ and $\mu(0,n,\Lam)$ has 
multiplicity two and every ``double'' eigenvalue $\mu(k_m,n,\Lam)$ 
with $m\neq0\ne n$ has multiplicity four with eigenfunctions $\psi_{\pm m\pm n}$.

(b) The eigenvalues $\mu(k_m,n,\Lam)$ do not explicitly depend on $\lam_1$, but implicitly. 
Recall that $\lam_1=\frac 1 2 \left( \frac 1 {2r^2} -2r\lam_2-2c_0^2\right)$, hence the parameters are not independent on the cylinder. 

(c) In the following we also use the notation $\Psi_{m,n}$ for the first 
two components of $\Psi_{m,n}$, which are the eigenvectors for the case 
of just the area constraint being active, cf.~Theorem \ref{exthm1} and 
\reff{areahelf} in \S\ref{cmr}. 

(d) The crucial difference of the spectrum of \reff{genev} and just the PDE part 
\reff{eigeq} is that $(\psi_{00},1,-2)$ with $\psi_{00}\equiv 1$ 
is not an eigenvector of $\pa_u\sG (0,\Lam)$. 
\eex\erem

\subsection{Center manifold construction}\label{cmr}
Based on the local existence Theorem \ref{exthm1} and the spectral 
computations from Lemma \ref{leig} we construct the center manifold 
for the flow near $\CC_L(r)$ which will be the basis for the subsequent 
stability and bifurcation results. 
At $\CC_L(r)$, $\det \CD=0$, and we cannot perturb $\CC_L(r)$ 
while preserving the area and the volume. Therefore we start with 
\hueq{\label{areahelf} \bpm \pa_t u\\ 0\epm = 
\bpm \eta^{-1}(u)G(u,\Lam)\\q_1(u,\Lam)\epm=:\CG_\CA(u,\Lam),}
where $\Lam=(\lam_1,\lam_2)$ with $\lam_2$ a {\em fixed} external 
pressure difference. 
The $\R^3$ has the Euclidean symmetry group $E(3)$ of rigid body motions, 
which can be constructed using two smooth curves 
$\tau,\brho:\R\ra\R^3$ with $\tau(0)=\brho(0)=0$, such that the translated and rotated surface is given by 
\hueqst{  
\tilde X=\{y+\tau(\eta)+y\times \brho(\eta): y\in X\}.
}
However, since we only consider normal variations of $X$, 
admissible rigid body motions are 
\hueqst{\CM X=\{X+u\, N: u =\spr{ \tau(\eta)+y\times \brho(\eta),N(y)}\}.} 
The dimension of $\CM X$ is given by the dimension of the tangent space 
$T_e \CM X$ at the identity, 
hence spanned by $\spr{\tau'(0),N(y)}$ and $\spr{y\times \brho'(0),N(y)}$. 
Since $\tau'(0)$ and $\brho'(0)$ are arbitrary vectors, 
\hueq{\label{ridmo}T_e\CM X=\mathrm{span} \{\spr{e_i,N},\spr{y\times e_i,N},\, i=1,2,3\}.} 
But for $\CC_L(r)$ we have 
\hueq{ \label{tcmfc} T_e \CM\Cr=\mathrm{span}\{ \spr{e_2,N}, \spr{e_3,N}\}=\mathrm{span}\{ \psi_{01}, \psi_{0-1}\}
}
where a straightforward calculation shows that translation in and 
rotation around $e_1$ generate tangential motions to $\CC_L(r)$, while 
rotations around $e_2$ and $e_3$ violate the periodicity in $x$. 

In \S\ref{stabrange} we will see that there are parameter values 
$\lam_2$ such that the spectrum of the linearization of \reff{areahelf} 
is contained in the negative half plane, with one zero eigenvalue 
with multiplicity according to \reff{tcmfc}. The spectrum on the finite 
cylinder is discrete, with a spectral gap between the zero and first non zero 
eigenvalue. Hence the spectrum decomposes into the center 
spectrum $\mathrm{spec}_c$ and the stable spectrum $\mathrm{spec}_s$. 
Using the well-posedness Theorem \ref{exthm1}  we may apply 
\cite[Theorem 4.1]{Si95} on the existence of a center manifold under 
the above conditions. Since \reff{tcmfc} shows that the center eigenspace 
coincides with the tangent space 
of the manifold of translated cylinders, both manifolds also coincide locally. 
This gives the following results, 
where again $y$ and $z$ are 
the euclidian coordinates orthogonal to the cylinder axis $x$. 
\blem\label{cmf}
At the trivial solution $(0,\lam_2)$ with $\lam_1$ and $\lam_2$ related by \reff{socon}, there exists a smooth center manifold $\mathcal M^c$ for \reff{areahelf} 
of dimension at least two. If the kernel of $\pa_{(u,\lam_2)}\CG_\CA$ 
is spanned by $\Psi_{0\pm1}$ then 
\hueq{\CM^c = \text{Shifts of $\CC_L$ in $y$ and $z$ direction}.}
\elem

\bthm\label{stabthm}
If $\lam_2\in\R$ such that the spectrum of $\pa_{(u,\lam_2)} \CG_\CA$ 
is contained in $(-\infty,0]$ and $\ker(\pa_{(u,\lam_2)} \CG_\CA)$ is spanned 
by $\Psi_{0\pm1}$, then there exists $\del,\om,M>0$ such that for all 
$u_0\in V^m_\eps$ with $\|u_0\|_{H^m}<\del$  
 the solution $U=(u,\lam_1)$ of \reff{areahelf} exists globally in time and 
there exist a unique $U_\infty\in \CM^c$ such that 
\hueqst{ \| U(t,U_0)-U_\infty\|_{H^m\times\R}\le Me^{-\om t}\|U_0\|_{H^m\times\R}.
} 
\ethm

\subsection{Stability and instability} \label{stabrange}
Following Theorem \ref{stabthm}, to check for stability of $\CC_L(r)$ 
we seek $\Lam\in\R^2$  such that all 
eigenvalues $\mu(k_m,n,\Lam)$ are in $(-\infty, 0]$, and the only 
zero eigenvalues belong to $\Psi_{0\pm1}$ (translations in $y$ and $z$).  
{\em From here on, to simplify notation we fix $r=1$}, and recall 
that the results for general $r$ follow from rescaling $r \mapsto 1$, 
$L\mapsto rL$ and $c_0\mapsto c_0/r$. 
Practically,  we vary $\lam_2$, with $\lam_1$ given by \reff{socon} 
along the trivial branch, and monitor the signs of eigenvalues. 
Depending on $c_0,L$, the main questions are:
\bci
\item Are there intervals for $\lam_2$ such that $\CC_L$ is linearly stable?
\item Which modes destabilize the cylinder at what $\lam_2$?
\eci 

In Lemma \ref{leig}, we fixed $L{>}0$ yielding the discrete allowed 
wave numbers $k_m=2\pi m/L$, $m\in\Z$. Analytically it is more convenient  
to return to continuous $k\in\R$. Thus we consider 
\huga{\label{mumu}
\mu(k,n,\lam_2)
=-\frac 1 2 (k^2+n^2)^2+(\lam_2+1)(k^2+n^2)-(\lam_2+1)-(1-2c_0)k^2, 
}
where due to the reflection (in $x$) 
symmetry of $\pa_u G(0)$ in \reff{Gjac} only even powers of $k$ appear, and 
hence we may restrict to $k\ge 0$, and similarly to $n\ge 0$. 
Subsequently we reintroduce 
$k_m$ to formulate  Corollary \ref{destabcor}. 
See also Fig.\ref{neigs} for illustration of the results. 

\input{neigs5}

For $k=0$ we have 
\huga{\label{azieig}
\mu(0,n,\lam_2)=-\frac{n^4}{2} +\left(\lam_2+1\right)n^2-\left(\lam_2+\frac1 2\right),}
with $\mu(0,1,\lam_2)=0$ for all $\lam_2$ (translational eigenvalues), and 
$\pa_{\lam_2} \mu(0,n,\lam_2)=n^2-1$
is positive for $n>1$. Furthermore $\mu$ is zero at 
$\lam_2^{(0,n)}=(1-n^2)^{-1}(-\frac{n^4}{2} +n^2-\frac 1 2)$, 
which is monotonically increasing in $n$. 
Hence, {\em under axially constant perturbations $\CC_L$ is stable for 
$\lam_2<\frac 3 2$}, 
indicated by the violet line in Fig.\ref{neigs}. 

% \input{neigs5}

Next we consider $k>0$ and $n\ne 0$, in particular  $n=1$ which 
turns out to be the most dangerous $n$ for $k\ne 0$. We have 
\hualst{\mu(k,1,\lam_2)&=-\frac 1 2 ((k^2+1)^2+(\lam_2+1)(k^2+1) 
-\left(\lam_2+\frac{1}{2}\right)-(1-2c_0)k^2\nonumber \\
&= -\frac 1 2 (k_1^2+1)^2 +(\lam_2+2c_0)k^2+\frac 1 2=-k^2(\frac 1 2 k^2+1-\lam_2-2c_0).
}
One sees directly that $\mu(k,1,\Lam)$ is strictly increasing 
in $\lam_2$ and has a zero at $k>0$ for 
\huga{\label{inmixed} 
\lam_2= \frac 1 2 k^2+1-2c_0,}
indicated by the yellow line in Fig.\ref{neigs}. In particular,  
{\em if $c_0>-1/4$, then there exists an explicitly computable 
$L$ large enough so that the $(k_1,1)$ coiling/buckling 
instability,  $k_1=2\pi/L$, 
in $\lam_2$ is below the wrinkling instability of $\CC_L$.} 

For $k>0$ and $n=0$ (pearling) 
we have, with $\kap:=k^2$, i.e., 
$\muti(\kap,\lam_2):=\mu(k^2,0,\lam_2)$, 
\hual{\label{l2p1} 
&\muti(\kap,\lam_2)=-\frac 1 2 \kap^2+(\lam_2+2c_0)\kap-\lam_2-\frac 1 2, 
%=0\\\aqui&\kap=\lam_2+2c_0\pm\sqrt{(\lam_2+2c_0)^2-2\lam_2-1}.
}
and solving $\mu(\kap,\lam_2)=0$ for $\lam_2=\lam_2(\kap)$ yields 
\huga{\label{l2hu}
\lam_2(\kap)=\frac 1 2 \frac{\kap^2-4c_0\kap+1}{\kap-1}=
\frac 1 2 (\kap-1)+\frac{(1-2c_0)\kap}{\kap-1}.
}
For $c_0\ne \frac 1 2$, this has a singularity at $\kap=1$ with 
\hugast{%\label{l2s}
\left\{\barr{ll} \lam_2(\kap)\to -\infty&\text{ if $\kap\nearrow 1$ and 
$c_0<1/2$, or $\kap\searrow 1$ and $c_0>1/2$},\\
\lam_2(\kap)\to \infty&\text{ if $\kap\nearrow 1$ and 
$c_0>1/2$, or $\kap\searrow 1$ and $c_0<1/2$}.
\earr\right.
}
For $c_0=\frac 1 2$ we have $\lam_2(\kap)=-1/2+\kap/2$. In any case, 
$\pa_{\lam_2}\muti(\kap,\lam_2)=\kap-1$ such that the unstable 
region is below $\lam_2(\kap)$ for $0<\kap<1$ and above 
$\lam_2(\kap)$ for $\kap>1$. See the blue curves/sets in Fig.\ref{neigs}. 
Finally, searching for extrema of $\lam_2(\kap)$ 
via $\pa_\kap \lam_2(\kap)=0$ yields 
\huga{\label{kape}
\kap_\pm=1\pm\sqrt{2-4c_0}.
} 
Hence, $\kap_\pm$ exist for $c_0<1/2$, and $\kap_-\in(0,1)$ for 
$c_0\in(1/4,1/2)$, and (only) in this case we {\em have a finite 
wave number $k=\sqrt{\kap}$ instability of $\CC_L$, for sufficiently 
large $L$}. 

Again, see Fig.\ref{neigs} (a)--(d) for illustration of these instability 
curves and selected dispersion relations, \huc{while in (e) we show 
the fully unstable case, which will be of interest for the outlook 
in Fig.\ref{c1f1}.}
In the following Corollary we summarize the 
above, with maximal wavelength refering to the minimal allowed 
$k_1=2\pi/L$. 

\bcor \label{destabcor}
The cylinder $\CC_L$ is volume and area preserving stable for every 
$L>0$ if:\\[-3mm]
\bcena
\item $c_0\in (1/4,1/2)$ and 
$\lam_2\in(\lam_2^{\text{pearl}},\lam_2^{\text{cb}})$ where 
$\lam_2^{\text{pearl}}=\lam_2(\kap_-)$ with $\kap_-=1-\sqrt{2-4c_0}$ 
and $\lam_2$ from \reff{l2hu},  and where $\lam_2^{\text{cb}}=1-2c_0$. 
In particular, $\CC_L$ with large $L$ destabilizes near 
$\lam_2^{\text{pearl}}$ to a finite wavelength 
pearling, and near $\lam_2^{\text{cb}}$ to 
maximal wavelength buckling and coiling. 
\item $c_0\in [-1/4,1/4]$ and $\lam_2\in(\lam_2^{\text{pearl}},\lam_2^{cb})$, 
where $\lam_2^{\text{pearl}}=-1/2$ and $\lam_2^{\text{cb}}=1-2c_0$. 
In particular, $\CC_L$ with large $L$ destabilizes near 
$\lam_2=-1/2$ to maximal wavelength pearling, and near 
$\lam_2^{\text{cb}}$ to maximal wavelength coiling and buckling.  
\item $c_0\in (-\infty,-1/4]$ and $\lam_2\in(\lam_2^{\text{pearl}},
\lam_2^{\text{wri}})$, where $\lam_2^{\text{pearl}}=-1/2$ and 
$\lam_2^{\text{wri}})=3/2$. In particular, 
$\CC_L$ with large $L$ destabilizes near $\lam_2=-1/2$ 
to maximal wavelength pearling, and at $\lam_2=3/2$ to 
wrinkling (homogeneous in $x$). 
\ecen
\vs{2mm}
If $c_0>1/2$, then for all $\lam_2\in\R$ there exists an $L_0>0$ such 
that $\CC_L$ with $L>L_0$ is spectrally unstable. 
\ecor

\huc{
\brem\label{carem}
The values $\lam_2^{\text{cb}}=1-2c_0$ and $\lam_2^\text{pearl}=-1/2$ 
are the asymptotics for $k_1\to 0$, i.e., for the infinitely 
long cylinder. In the following section we return to some finite 
$L>0$, i.e., some finite $k_1=2\pi/L$, and in the numerics in \S\ref{numex} 
we use, e.g., $L=10$, hence $k_1=\pi/5\approx 0.628$, or 
$L=30$, hence $k_1=\pi/15\approx 0.209$. The corresponding values 
for  $\lam_2^{\text{cb}}$ and $\lam_2^\text{pearl}$ (maximum wavelength 
pearling) can then be read off from the orange and blue lines 
in Fig.\ref{neigs}. For, e.g., $c_0=0.48$ and $L=30$, 
the finite wavelength pearling 
corresponds to $k_m=2\pi m/30\approx 0.838$ for $m=4$. 
\eex\erem 
}


==> stcyb1.tex <==
\section{Stability of $\CC_L$}\label{stcy}
We consider the linearization of \reff{hflow} around $\CC_L(r)$. 
This requires some lengthy computations, but since $\CC_L(r)$ has 
constant mean and Gaussian curvatures (with $K=0$), we can explicitly 
compute the 
dispersion relation (Lemma \ref{leig}) and subsequently the stability ranges 
of and bifurcation points from $\CC_L(r)$ (Corollary \ref{destabcor}).
\subsection{Linearization and eigenvalues}\label{lineig}
Since $G(\cdot,\Lam):V^4_\eps\to L^2$ is an analytic map, 
we use \reff{meanu}, \reff{gaussu} and \reff{LBu} to calculate the 
Frech\'et derivative via the Gateaux differential in direction $v$, i.e., 
$\pa_u G(0,\Lam)v=\frac{\dd}{\dd \eps} G(\eps v,\Lam)|_{\eps=0}$; recall that  the Laplace-Beltrami operator on $\CC_L((r)$ is $\Delta_0=\pa_x^2+\frac 1 {r^2} \pa_\bphi^2$ in our coordinate system.
\blem \label{dcomp} The linearizations of 
$H(u), K(u)$, and $\Delta_uH(u)$ around $\CC_L(r)$, i.e., around $u=0$, 
are given by 
\hual{\label{dmean}\pa_u H(0)v&=-\frac 1 2\left(\Delta_0v +\frac 1 {r^2} v\right),\\
\label{dgauss}\pa_uK(0) v&=-r^{-1} \pa_x^2 v, \text{ and }\\[2mm]
\label{dlead}\pa_u \Delta_0H(0)v &= \Delta \pa_u H(0)v.
}
\elem
\begin{proof}
Using \reff{meanu} with $\eps v$ %and sorting by $\eps$ powers 
gives
\hueqst{ 2H(\eps v)=-\frac{\eps(r^3 v_{xx}+rv_{\bphi\bphi}) +\CO(\eps^2)}{(r^2+\eps 2rv+\CO(\eps^2))^{3/2}}+\frac{1}{(r^2+\eps 2rv+\CO(\eps^2))^{1/2}}.}
Differentiating wrt $\eps$ this gives 
\hueqst{\frac{\dd}{\dd \eps} 2 H(\eps v)=-\frac{(r^3 v_{xx}+rv_{\bphi\bphi})(r^2+\CO(\eps))^{3/2}+\CO(\eps)}{(r^2+\eps 2rv+\CO(\eps^2))^{3}}-\frac{r v+\CO(\eps)}{(r^2+\CO(\eps))^{3/2}}.}

The denominators are bounded away from zero, hence evaluating at $\eps=0$ gives \reff{dmean}.

For $K$ this works the same way, with 
\hueqst{ \frac{\dd}{\dd \eps} K(\eps v)= \frac{\dd}{\dd \eps}  \frac{-\eps r^3 v_{xx} +\CO(\eps^2)}{(r^2+2\eps 2rv+\CO(\eps^2))^2}=\frac{-r^3 v_{xx} ((r^2+\eps 2rv+O(\eps^2))^{2} +\CO(\eps)}{(r^2+\eps 2rv+\CO(\eps^2))^{4}}.}
Again evaluating at $\eps=0$ gives \reff{dgauss}. 

Finally for \reff{dlead} it is sufficient to notice that 
\hueqst{\frac{\dd}{\dd \eps} \Delta_{\eps v}H(\eps v)|_{\eps=0} = \left(\frac{\dd}{\dd \eps}\Delta_{\eps v} H(0)\right)\bigg|_{\eps=0} +\Delta_0  \left(\frac{\dd}{\dd \eps}H(\eps v)\bigg|_{\eps=0}\right)=\Delta_0  \left(\frac{\dd}{\dd \eps}H(\eps v)\bigg|_{\eps=0}\right),}
since $H(0)$ is a constant and $\Delta_{\eps v}$ is non degenerate for small perturbations. 
\end{proof}

Inserting the expressions from Lemma \ref{dcomp} we obtain 
\blem $G(\cdot,\Lam)$ is Frechet differentiable at $u=0$, with differential, 
using \reff{socon}, 
\hual{\label{Gjac} \pa_uG(0,\Lam) v= -\frac 1 2\Delta^2_0 v-\left(r\lam_2+\frac{1}{r^2}\right) \Delta_0 v- \left(\frac{\lam_2}{r} +\frac{1}{2r^4}\right) v +\left(\frac 1 r-2c_0\right) r^{-1} \pa_x^2 v.
}
\elem
Over the unbounded $\CC(r)$, $\pa_uG(0,\Lam))$ has a continuous spectrum, 
but by restricting to the compact cylinder $\CC_L(r)$ of length $L$, 
 $\pa_uG(0,\Lam))$ has a discrete spectrum with a simple basis 
of eigenfunctions. 
\blem \label{leig}
The eigenvalue equation 
\hueq{ \label{eigeq}\pa_uG(0,\Lam)\psi=\mu\psi}
has a countable set of solutions $(\mu_{mn},\psi_{mn})\in 
\R\times H^4_{\per}(\CC_L(r))$,  $(m,n)\in\Z^2$, 
\bsub\label{eigs}
\hual{
&\text{$\psi_{mn}(x,\bphi)=e^{\ri (k_mx+n\bphi)}$, 
$k_m=2m\pi/L$, with}\\
%\hual{\label{eigs} 
&\mu(m,n,\Lam)=-\frac 1 2  \Big[k_m^2+\frac {n^2} {r^2} \Big]^2 +\left(r\lam_2+\frac{1}{r^2}\right)\Big[k_m^2+\frac {n^2} {r^2} \Big]&- \left(\frac{\lam_2}{r} +\frac{1}{2r^4}\right) -\left(\frac 1 r-2c_0\right) \frac{ k_m^2}{r}.
}
\esub 
For all $\Lam\in\R^2$ the eigenfunctions $\psi_{0\pm1} \in\ker(\pa_uG(0,\Lam))$.
\elem
\begin{proof}
Recall that $H^4_{\per}(\CC_L(r))$ has a compact embedding in $L^2(\CC_L(r))$, 
hence the resolvent of \reff{Gjac} is compact. Using the $L^2$ basis of 
eigenfunctions of $\Delta_0$, 
\hueqst{ \psi_{mn}(x,\bphi)=e^{\ri(k_mx+n\bphi)}, \quad 
\Delta_0\psi_{mn}= -\Big[k_m^2+\frac 1 {r^2} n^2\Big]\psi_{mn}(x,\bphi), 
}
we obtain 
$\mu=
-\frac 1 2  \Big[k_m^2+\frac 1 {r^2}n^2\Big]^2 
+\left(r\lam_2+\frac{1}{r^2}\right)\Big[k_m^2+\frac 1 {r^2} n^2\Big]
- \left(\frac{\lam_2}{r} +\frac{1}{2r^4}\right) 
-\frac 1 r\left(\frac 1 r-2c_0\right) r^{-1} k_m^2$, 
hence \reff{eigs} after some rearranging. 
Clearly $\mu(0,\pm1,\Lam)=0$, hence 
$\psi_{0\pm1}\in \ker(\pa_uG(0,\Lam))$. 
\end{proof}
Using Lemma \ref{aderlem}, we write the linearization of \reff{hflowu} as 
\hual{ \label{genev0}\pa_U \sG(0,\Lam) U
& =\bpm \pa_u G(0,\Lam ) & \pa_{\lam_1} G(0,\Lam ) &\pa_{\lam_2} G(0,\Lam ) \\ 
		\pa_u \CA(0 ) & \pa_{\lam_1} \CA(0 ) &\pa_{\lam_2} \CA(0 )\\
		\pa_u \CV(0 ) & \pa_{\lam_1} \CV(0 ) &\pa_{\lam_2} \CV(0 )
		 \epm  \bpm u\\ \sig_1\\\sig_2\epm\nonumber\\
	&=\bpm \pa_u G(0,\Lam )u & -2H(0) \sig_1&-\sig_2 \\ 
		-\int_{\CC_L(r)} 2H(0) u\dd S &0 & 0\\
		\int_{\CC_L(r)} u \dd S& 0 & 0
\epm.}
The domain of $\pa_U\CG(0,\Lam)$ is $H^4_\per(\CC_L(r))\times \R^2$,  
equipped with the norm $\|U\|_{\pa_{(u,\Lam)}\sG}=\|u\|_{H^4}+\|\Sigma\|_{\R^2}$, and altogether we have the generalized eigenvalue problem 
 $\Psi=(\psi,\sig_1,\sig_2)$
\hual{ \label{genev}\pa_U \sG(0,\Lam) \Psi
= \mu \bpm 1 & 0& 0\\0 & 0& 0\\0 & 0& 0 \epm \Psi,}
with eigenvalues $\mu \in \{ \nu(m,n), \, (m,n)\in\Z^2\backslash \{(0,0)\}\cup \{0\}$ and eigenfunctions 
\hueqst{\Psi_{m,n}= \bpm \psi_{m,n}\\ 1\\ -2\epm, \, (m,n)\in\Z^2\backslash \{(0,0)\}, \text{ and }\Psi_{0,0}=\bpm 0\\ 1\\ -2\epm.
} 
\brem (a) The eigenvalues $\mu(0,\pm 1,\lam)=0$ correspond to 
translations of $\CC_L(r)$ in $y$ and $z$ directions. 
 Each eigenvalue of the form $\mu(m,0,\Lam)$ and $\mu(0,n,\Lam)$ has 
multiplicity two and every ``double'' eigenvalue $\mu(m,n,\Lam)$ 
with $m\neq0\ne n$ has multiplicity four with eigenfunctions $\psi_{\pm m\pm n}$.

(b) The eigenvalues $\mu(m,n,\Lam)$ do not explicitly depend on $\lam_1$, but implicitly. Recall \reff{socon}, i.e., 
$\lam_1=\frac 1 2 \left( \frac 1 {2r^2} -2r\lam_2-2c_0^2\right)$, hence the parameters are not independent on the cylinder. 

(c) In the following we also use the notation $\Psi_{m,n}$ for the first 
two components of $\Psi_{m,n}$, which are the eigenvectors for the case 
of just the area constraint being active, cf.~Theorem \ref{exthm1} and 
\reff{areahelf} in \S\ref{cmr}. 

(d) The crucial difference of the spectrum of \reff{genev} and just the PDE part 
\reff{eigeq} is that $(\psi_{00},1,-2)$ with $\psi_{00}\equiv 1$ 
is not an eigenvector of $\pa_u\sG (0,\Lam)$. 
\eex\erem

\subsection{Center manifold construction}\label{cmr}
Based on the local existence Theorem \ref{exthm1} and the spectral 
computations from Lemma \ref{leig} we construct the center manifold 
for the flow near $\CC_L(r)$ which will be the basis for the subsequent 
stability and bifurcation results. 
At $\CC_L(r)$, $\det \CD=0$, and we cannot perturb $\CC_L(r)$ 
while preserving the area and the volume. Therefore we start with 
\hueq{\label{areahelf} \bpm \pa_t u\\ 0\epm = 
\bpm \eta^{-1}(u)G(u,\Lam)\\q_1(u,\Lam)\epm=:\CG_\CA(u,\Lam),}
where $\Lam=(\lam_1,\lam_2)$ with $\lam_2$ a {\em fixed} external 
pressure difference. 
The $\R^3$ has the Euclidean symmetry group $E(3)$ of rigid body motions, 
which can be constructed using two smooth curves 
$\tau,\brho:\R\ra\R^3$ with $\tau(0)=\brho(0)=0$, such that the translated and rotated surface is given by 
\hueqst{  
\tilde X=\{y+\tau(\eta)+y\times \brho(\eta): y\in X\}.
}
However, since we only consider normal variations of $X$, 
admissible rigid body motions are 
\hueqst{\CM X=\{X+u\, N: u =\spr{ \tau(\eta)+y\times \brho(\eta),N(y)}\}.} 
The dimension of $\CM X$ is given by the dimension of the tangent space 
$T_e \CM X$ at the identity, 
hence spanned by $\spr{\tau'(0),N(y)}$ and $\spr{y\times \brho'(0),N(y)}$. 
Since $\tau'(0)$ and $\brho'(0)$ are arbitrary vectors, 
\hueq{\label{ridmo}T_e\CM X=\mathrm{span} \{\spr{e_i,N},\spr{y\times e_i,N},\, i=1,2,3\}.} 
But for $\CC_L(r)$ we have 
\hueq{ \label{tcmfc} T_e \CM\Cr=\mathrm{span}\{ \spr{e_2,N}, \spr{e_3,N}\}=\mathrm{span}\{ \psi_{01}, \psi_{0-1}\}
}
where a straightforward calculation shows that translation in and 
rotation around $e_1$ generate tangential motions to $\CC_L(r)$, while 
rotations around $e_2$ and $e_3$ violate the periodicity in $x$. 
%assumption on $u$. 

In \S\ref{stabrange} we will see that there are parameter values 
$\lam_2$ such that the spectrum of the linearization of \reff{areahelf} 
is contained in the negative half plane, with one zero eigenvalue 
with multiplicity according to \reff{tcmfc}. The spectrum on the finite 
cylinder is discrete, with a spectral gap between the zero and first non zero 
eigenvalue. Hence the spectrum decomposes into the center 
spectrum $\mathrm{spec}_c$ and the stable spectrum $\mathrm{spec}_s$. 
Using the well-posedness Theorem \ref{exthm1}  we may apply 
\cite[Theorem 4.1]{Si95} on the existence of a center manifold under 
the above conditions. Since \reff{tcmfc} shows that the center eigenspace 
coincides with the tangent space 
of the manifold of translated cylinders, both manifolds also coincide locally. 
This gives the following results, where again $y$ and $z$ are 
the euclidian coordinates orthogonal to the cylinder axis $x$. 
\blem\label{cmf}
At the trivial solution $(0,\lam_2)$ with $\lam_1$ and $\lam_2$ related by \reff{socon}, there exists a smooth center manifold $\mathcal M^c$ for \reff{areahelf} 
of dimension at least two. If the kernel of $\pa_{(u,\lam_2)}\CG_\CA$ 
is spanned by $\Psi_{0\pm1}$ then 
\hueq{\CM^c = \text{Shifts of $\CC_L$ in $y$ and $z$ direction}.}
\elem


\bthm\label{stabthm}
If $\lam_2\in\R$ such that the spectrum of $\pa_{(u,\lam_2)} \CG_\CA$ 
is contained in $(-\infty,0]$ and $\ker(\pa_{(u,\lam_2)} \CG_\CA)$ is spanned 
by $\Psi_{0\pm1}$, then there exists $\del,\om,M>0$ such that for all 
$u_0\in V^m_\eps$ with $\|u_0\|_{H^m}<\del$  
 the solution $U=(u,\lam_1)$ of \reff{areahelf} exists globally in time and 
there exists a unique $U_\infty\in \CM^c$ such that 
\hueqst{ \| U(t,U_0)-U_\infty\|_{H^m\times\R}\le Me^{-\om t}\|U_0\|_{H^m\times\R}.
} 
\ethm

\subsection{Stability and instability} \label{stabrange}
Following \autoref{stabthm}, to check for stability of $\CC_L(r)$ 
we seek $\Lam\in\R^2$  such that all 
eigenvalues $\mu(m,n,\Lam)$ are in $(-\infty, 0]$, and the only 
zero eigenvalues belong to $\Psi_{0\pm1}$ (translations in $y$ and $z$).  
{\em From here on, to simplify notation we fix $r=1$}, and recall 
that the results for general $r$ follow from rescaling $r \mapsto 1$, 
$L\mapsto rL$ and $c_0\mapsto c_0/r$. 
Practically,  we vary $\lam_2$ along the trivial branch, and monitor the 
signs of the eigenvalues. Due to the three parameters $(L,c_0,\lam_2)$, 
with $\lam_1$ given by \reff{socon}, we will 
distinguish between several cases, while the main questions are:
\bci
\item Are there intervals for $\lam_2$ such that $\CC_L$ is linearly stable?
\item Which modes destabilize the cylinder at what $\lam_2$?
\eci 
The zeros of $\mu$ give values $\lam_2(m,n)$, indicating which mode 
induces the instability. 
Thus we compute the zeros of $\mu(m,n,\Lam)$ and the slope 
$\pa_{\lam_2}\mu(m,n,\Lam)$,  
giving us on which side the eigenvalue is negative, splitting the 
$(L,c_0)$ plane. As a visualization, \autoref{neigs} shows plots of the 
regions of stability (in green) and some spectral plots of selected 
dispersion relations. 

For $m=0$ we have 
\hueq{\label{azieig}\mu(0,n,\Lam)=-\frac{n^4}{2} +\left(\lam_2+1\right)n^2-\left(\lam_2+\frac1 2\right),}
with $\mu(0,\pm 1,\Lam)=0$ for all $\Lam$ (translational eigenvalues), and 
$\pa_{\lam_2} \mu(0,n,\Lam)=n^2-1$
is positive for $n>1$. Furthermore $\mu$ is zero at
\hueq{\label{azil}
\lam_2^{(0,n)}:=(1-n^2)^{-1}(-\frac{n^4}{2} +n^2-\frac 1 2),}
which is monotonically increasing in $n$. 
Hence {\em under axially constant perturbations $\Cr$ is stable for $\lam_2<\frac 3 2$.} 

 \input{neigs2}


Next we consider the modes $m\ne 0\ne n$, in particular  $(m,n)=(1,1)$, where 
\hualst{\mu(1,1,\Lam)&=-\frac 1 2 ((k_1^2+1)^2+(\lam_2+1)(k_1^2+1) 
-\left(\lam_2+\frac{1}{2}\right)-(1-2c_0)k_1^2\nonumber \\
&= -\frac 1 2 (k_1^2+1)^2 +(\lam_2+2c_0)k_1^2+\frac 1 2.}
One sees directly that $\mu(1,1,\Lam)$ is strictly increasing 
in $\lam_2$ and has a zero for 
\hueq{\label{inmixed} \lam_2^{(1,1)}:= \frac 1 2 k_1^2+1-2c_0,}
where $\lam_2$ is strictly decreasing in $L$ because so is $k_m=2m\pi/L$. 
Hence, 
{\em if $c_0>-1/4$, then there exists an $L$ large enough so that the cylinder destabilizes due to the $(m,n)=(1,1)$ mode with $L$ explicitly computable.}

For $m\geq1$ and $n=0$ (pearling), the eigenvalues 
\hueqst{ 
\mu(m,0,\Lam)=-\frac 1 2 k_m^4+(\lam_2+2c_0)k_m^2-\lam_2-\frac 1 2
}
behave as follows. Depending on $L$, 
either $k_m<1$  such that $\mu(m,0,\Lam)$ is strictly decreasing in $\lam_2$, or 
$k_m>1$  such that $\mu(m,0,\Lam)$ is strictly increasing in $\lam_2$. 
In either case, for $m=1$ the eigenvalue has a zero at 
\hueq{\label{perbp}\lam_2^{(m,0)}
:=\Big[1-k_m^2\Big]^{-1} \Bigg(-\frac 1 2 k_m^4 +2c_0k_m^2 - \frac 1 2 \Bigg)}
for all $L\in\R\backslash\{2\pi m\}$. 
First we note that the asymptote at $L=2\pi m$ is odd, where for $c_0<\frac m 2$, $\lim_{k_m\searrow 1}\lam_2=-\infty$ and for $c_0>\frac m 2$ the other way around. In the latter case there always exists a $L$ such that the $m$'th mode destabilizes the cylinder, so we do not focus further on that case. 
A straightforward analysis of \reff{perbp} shows that it admits 
two positive solutions 
\hueqst{ 
L= \begin{cases} 
L_G=2\pi\left(\frac{1+ \sqrt{2}\sqrt{1-2c_0}}{4c_0-1}\right)^{1/2}  
\quad\text{ for } c_0\in(1/4,1/2],\\
L_{S_1}=2\pi\left(\frac{1- \sqrt{2}\sqrt{1-2c_0}}{4c_0-1}\right) 
\quad\text{ for } c_0\in(-\infty,1/2],\\
L_{S_2}=\sqrt{2} \pi, \hs{20mm}\text {for } c_0=1/4, 
\end{cases}
}
where for $i=1,2$ it holds that $L_{S_i}<2\pi$ and are minima. 
For $c_0\leq \frac 1 2$ and $L>2\pi$ the eigenvalue $\mu(1,0,\Lam)$ has negative slope at \reff{perbp}, hence for smaller $\lam_2$ the cylinder is destabilized. 
In the case of $c_0\leq \frac 1 4$, $\lam_2$ is monotonically increasing 
in $L$, yielding a maximum wavelength instability. 
In the regime where $L_G$ exists, the $\CC_L$ destabilizes to a finite 
wave length. 

In the following Corollary of \autoref{stabthm} we summarize the above, where 
maximal wave length (or long wave instability) refers to the minimal allowed 
$k_1=2\pi/L$, since $k_0=0$ is prohibited by the volume and area constraints. 
\bcor \label{destabcor}
The cylinder $\CC_L$ is volume and area preserving stable for every $L>0$ if, 
with constants $\lam_2^{m,n}$ given in \reff{azil}--\reff{perbp}:\\[-3mm]
\bcena
\item $c_0\in (1/4,1/2)$ and $\lam_2\in(\lam_2^{(1,0)},\lam_2^{(1,1)})$; 
$\CC_L$ destabilizes at $ \lam_2^{(1,0)}$ with finite wave length $L_G$ wrt 
the mode $\psi_{20}$ (pearling), and at $\lam_2^{(1,1)}$ wrt 
the mode $\psi_{11}$ (buckling and coiling) of maximal wave length. 
\item $c_0\in [-1/4,1/4]$ and $\lam_2\in(\lam_2^{(1,0)},\lam_2^{(1,1)})$; $\CC_L$  destabilizes at $ \lam_2^{(1,0)}$ wrt to the mode $\psi_{10}$ (pearling), 
and at 
$\lam_2^{(1,1)}$ wrt the mode $\psi_{11}$ (buckling and coiling), both of maximal 
wave length. 
\item $c_0\in (-\infty,-1/4]$ and $\lam_2\in(\lam_2^{(1,0)},\lam_2^{(0,2)})$; 
$\CC_L$ destabilizes at $ \lam_2^{(1,0)}$ wrt the mode $\psi_{10}$ (pearling)  
with maximal wave length, and at $\lam_2^{(0,2)}$ wrt the mode $\psi_{01}$ 
(wrinkling, homogeneous in $x$). 
\ecen
\vs{2mm}
If $c_0>1/2$ there is always a positive eigenvalue for every $\lam_2$, hence the cylinder is spectrally unstable. 
\ecor

